Reflective Decoding: Beyond Unidirectional Generation with Off-the-Shelf Language Models

Publicly available, large pretrained LanguageModels (LMs) generate text with remarkable quality, but only sequentially from left to right. As a result, they are not immediately applicable to generation tasks that break the unidirectional assumption, such as paraphrasing or text-infilling, necessitating task-specific supervision. In this paper, we present Reflective Decoding, a novel unsupervised algorithm that allows for direct application of unidirectional LMs to non-sequential tasks. Our 2-step approach requires no supervision or even parallel corpora, only two off-the-shelf pretrained LMs in opposite directions: forward and backward. First, in the contextualization step, we use LMs to generate ensembles of past and future contexts which collectively capture the input (e.g. the source sentence for paraphrasing). Second, in the reflection step, we condition on these "context ensembles", generating outputs that are compatible with them. Comprehensive empirical results demonstrate that Reflective Decoding outperforms strong unsupervised baselines on both paraphrasing and abductive text infilling, significantly narrowing the gap between unsupervised and supervised methods. Reflective Decoding surpasses multiple supervised baselines on various metrics including human evaluation.

==> bib_backup.tex <==
% Please download the latest anthology.bib from
%
% http://aclweb.org/anthology/anthology.bib.gz

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}


% BELOW IS ALL PULLED FROM THE EMNLP SUBMISSION

@article{harris1954distributional,
  title={Distributional structure},
  author={Harris, Zellig S},
  journal={Word},
  volume={10},
  number={2-3},
  pages={146--162},
  year={1954},
  publisher={Taylor \& Francis}
}

@inproceedings{see2017get,
  title={Get To The Point: Summarization with Pointer-Generator Networks},
  author={See, Abigail and Liu, Peter J and Manning, Christopher D},
  booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={1073--1083},
  year={2017}
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@inproceedings{hashimoto2019unifying,
  title={Unifying Human and Statistical Evaluation for Natural Language Generation},
  author={Hashimoto, Tatsunori and Zhang, Hugh and Liang, Percy},
  booktitle={Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
  pages={1689--1701},
  year={2019}
}

@inproceedings{du2019empirical,
  title={An Empirical Comparison on Imitation Learning and Reinforcement Learning for Paraphrase Generation},
  author={Du, Wanyu and Ji, Yangfeng},
  booktitle={Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)},
  pages={6014--6020},
  year={2019}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  pages={5998--6008},
  year={2017}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@inproceedings{khandelwal2018sharp,
  title={Sharp Nearby, Fuzzy Far Away: How Neural Language Models Use Context},
  author={Khandelwal, Urvashi and He, He and Qi, Peng and Jurafsky, Dan},
  booktitle={Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={284--294},
  year={2018}
}

@inproceedings{roy2019unsupervised,
  title={Unsupervised Paraphrasing without Translation},
  author={Roy, Aurko and Grangier, David},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={6033--6039},
  year={2019}
}

@inproceedings{peters2018deep,
  title={Deep Contextualized Word Representations},
  author={Peters, Matthew and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)},
  pages={2227--2237},
  year={2018}
}

@inproceedings{conneau2019cross,
  title={Cross-lingual Language Model Pretraining},
  author={Conneau, Alexis and Lample, Guillaume},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7057--7067},
  year={2019}
}

@article{radford2018improving,
  title={Improving language understanding by generative pre-training},
  author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya}
}

@inproceedings{gururangan2018annotation,
  title={Annotation Artifacts in Natural Language Inference Data},
  author={Gururangan, Suchin and Swayamdipta, Swabha and Levy, Omer and Schwartz, Roy and Bowman, Samuel and Smith, Noah A},
  booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 2 (Short Papers)},
  pages={107--112},
  year={2018}
}

@inproceedings{devlin2019bert,
  title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  booktitle={Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
  pages={4171--4186},
  year={2019}
}

@article{liu2019roberta,
  title={Roberta: A robustly optimized bert pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}

@inproceedings{kiros2015skip,
  title={Skip-thought vectors},
  author={Kiros, Ryan and Zhu, Yukun and Salakhutdinov, Russ R and Zemel, Richard and Urtasun, Raquel and Torralba, Antonio and Fidler, Sanja},
  booktitle={Advances in neural information processing systems},
  pages={3294--3302},
  year={2015}
}

@article{firth1957synopsis,
  title={A synopsis of linguistic theory, 1930-1955},
  author={Firth, John R},
  journal={Studies in linguistic analysis},
  year={1957},
  publisher={Basil Blackwell}
}


@book{Aho:72,
    author  = {Alfred V. Aho and Jeffrey D. Ullman},
    title   = {The Theory of Parsing, Translation and Compiling},
    year    = "1972",
    volume  = "1",
    publisher = {Prentice-Hall},
    address = {Englewood Cliffs, NJ}
}

@book{APA:83,
    author  = {{American Psychological Association}},
    title   = {Publications Manual},
    year    = "1983",
   publisher = {American Psychological Association},
   address = {Washington, DC}
}

@article{Chandra:81,
	author = {Ashok K. Chandra and Dexter C. Kozen and Larry J. Stockmeyer},
	year = "1981",
	title = {Alternation},
	journal = {Journal of the Association for Computing Machinery},
	volume = "28",
	number = "1",
	pages = "114--133",
	doi = "10.1145/322234.322243",
}

@inproceedings{andrew2007scalable,
  title={Scalable training of {L1}-regularized log-linear models},
  author={Andrew, Galen and Gao, Jianfeng},
  booktitle={Proceedings of the 24th International Conference on Machine Learning},
  pages={33--40},
  year={2007},
}

@book{Gusfield:97,
    author  = {Dan Gusfield},
    title   = {Algorithms on Strings, Trees and Sequences},
    year    = "1997",
    publisher = {Cambridge University Press},
    address = {Cambridge, UK}
}

@article{rasooli-tetrault-2015,
    author    = {Mohammad Sadegh Rasooli and Joel R. Tetreault},
    title     = {Yara Parser: {A} Fast and Accurate Dependency Parser},
    journal   = {Computing Research Repository},
    volume    = {arXiv:1503.06733},
    year      = {2015},
    url       = {http://arxiv.org/abs/1503.06733},
    note    = {version 2}
}

@article{Ando2005,
	Acmid = {1194905},
	Author = {Ando, Rie Kubota and Zhang, Tong},
	Issn = {1532-4435},
	Issue_Date = {12/1/2005},
	Journal = {Journal of Machine Learning Research},
	Month = dec,
	Numpages = {37},
	Pages = {1817--1853},
	Publisher = {JMLR.org},
	Title = {A Framework for Learning Predictive Structures from Multiple Tasks and Unlabeled Data},
	Volume = {6},
	Year = {2005}}

%%%%%%
% My citations
%%%%%%

% baselines

@inproceedings{DiPS2019,
  title={Submodular Optimization-based Diverse Paraphrasing and its Effectiveness in Data Augmentation},
  author={Ashutosh Kumar and Satwik Bhattamishra and Manik Bhandari and Partha Talukdar},
  booktitle={NAACL-HLT},
  year={2019}
}

@inproceedings{WYU2019,
  title={An Empirical Comparison on Imitation Learning and Reinforcement Learning for Paraphrase Generation},
  author={Wanyu Du and Yangfeng Ji},
  booktitle={EMNLP/IJCNLP},
  year={2019}
}

@inproceedings{Roy2019,
  title={Unsupervised Paraphrasing without Translation},
  author={Aurko Roy and David Grangier},
  booktitle={ACL},
  year={2019}
}

@article{Gupta2018DeepGenFramework,
  title={A Deep Generative Framework for Paraphrase Generation},
  author={Ankush Gupta and Arvind Agarwal and Prawaan Singh and Piyush Rai},
  journal={ArXiv},
  year={2018},
  volume={abs/1709.05074}
}


@inproceedings{Li2018DeepRL,
  title={Paraphrase Generation with Deep Reinforcement Learning},
  author={Zichao Li and Xin Jiang and Lifeng Shang and Huang Li},
  booktitle={EMNLP},
  year={2018}
}

@inproceedings{Yang2019E2E,
  title={An End-to-End Generative Architecture for Paraphrase Generation},
  author={Qian Yang and Zhouyuan Huo and Dinghan Shen and Yong Cheng and Wenlin Wang and Guoyin Wang and Lawrence Carin},
  booktitle={EMNLP/IJCNLP},
  year={2019}
}

@inproceedings{Li2019DecomposableNP,
  title={Decomposable Neural Paraphrase Generation},
  author={Zichao Li and Xin Jiang and Lifeng Shang and Qun Liu},
  booktitle={ACL},
  year={2019}
}

@article{lewis2019bart,
  title={Bart: Denoising sequence-to-sequence pre-training for natural language generation, translation, and comprehension},
  author={Lewis, Mike and Liu, Yinhan and Goyal, Naman and Ghazvininejad, Marjan and Mohamed, Abdelrahman and Levy, Omer and Stoyanov, Ves and Zettlemoyer, Luke},
  journal={arXiv preprint arXiv:1910.13461},
  year={2019}
}

@misc{word2vec,
title	= {Efficient Estimation of Word Representations in Vector Space},
author	= {Tomas Mikolov and Kai Chen and Greg S. Corrado and Jeffrey Dean},
year	= {2013},
URL	= {http://arxiv.org/abs/1301.3781}
}



% tasks

@article{Bhagavatula2019AbductiveCR,
  title={Abductive Commonsense Reasoning},
  author={Chandra Bhagavatula and Ronan Le Bras and Chaitanya Malaviya and Keisuke Sakaguchi and Ari Holtzman and Hannah Rashkin and Doug Downey and Scott Yih and Yejin Choi},
  journal={ICLR},
  year={2020}
}

@inproceedings{TREC,
  title={Learning question classifiers},
  author={Li, Xin and Roth, Dan},
  booktitle={Proceedings of the 19th international conference on Computational linguistics-Volume 1},
  pages={1--7},
  year={2002},
  organization={Association for Computational Linguistics}
}

@article{coucke2018snips,
  title={Snips voice platform: an embedded spoken language understanding system for private-by-design voice interfaces},
  author={Coucke, Alice and Saade, Alaa and Ball, Adrien and Bluche, Th{\'e}odore and Caulier, Alexandre and Leroy, David and Doumouro, Cl{\'e}ment and Gisselbrecht, Thibault and Caltagirone, Francesco and Lavril, Thibaut and others},
  journal={arXiv preprint arXiv:1805.10190},
  year={2018}
}


@inproceedings{qian-etal-2019-diversepara,
    title = "Exploring Diverse Expressions for Paraphrase Generation",
    author = "Qian, Lihua  and
      Qiu, Lin  and
      Zhang, Weinan  and
      Jiang, Xin  and
      Yu, Yong",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D19-1313",
    doi = "10.18653/v1/D19-1313",
    pages = "3173--3182",
}


@inproceedings{miao2019cgmh,
  title={Cgmh: Constrained sentence generation by metropolis-hastings sampling},
  author={Miao, Ning and Zhou, Hao and Mou, Lili and Yan, Rui and Li, Lei},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={6834--6842},
  year={2019}
}


@inproceedings{bao2019dss,
  title={Generating Sentences from Disentangled Syntactic and Semantic Spaces},
  author={Bao, Yu and Zhou, Hao and Huang, Shujian and Li, Lei and Mou, Lili and Vechtomova, Olga and Dai, Xinyu and Chen, Jiajun},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={6008--6019},
  year={2019}
}

@article{liu2019upsa,
  title={Unsupervised Paraphrasing by Simulated Annealing},
  author={Liu, Xianggen and Mou, Lili and Meng, Fandong and Zhou, Hao and Zhou, Jie and Song, Sen},
  journal={arXiv preprint arXiv:1909.03588},
  year={2019}
}

% metrics

@inproceedings{lin-2004-rouge,
    title = "{ROUGE}: A Package for Automatic Evaluation of Summaries",
    author = "Lin, Chin-Yew",
    booktitle = "Text Summarization Branches Out",
    month = jul,
    year = "2004",
    address = "Barcelona, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W04-1013",
    pages = "74--81",
}

@inproceedings{papineni2002bleu,
  title={BLEU: a method for automatic evaluation of machine translation},
  author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
  booktitle={Proceedings of the 40th annual meeting on association for computational linguistics},
  pages={311--318},
  year={2002},
  organization={Association for Computational Linguistics}
}

@inproceedings{denkowski2014meteor,
  title={Meteor universal: Language specific translation evaluation for any target language},
  author={Denkowski, Michael and Lavie, Alon},
  booktitle={Proceedings of the ninth workshop on statistical machine translation},
  pages={376--380},
  year={2014}
}

@article{snover2009ter,
  title={TER-Plus: paraphrase, semantic, and alignment enhancements to Translation Edit Rate},
  author={Snover, Matthew G and Madnani, Nitin and Dorr, Bonnie and Schwartz, Richard},
  journal={Machine Translation},
  volume={23},
  number={2-3},
  pages={117--127},
  year={2009},
  publisher={Springer}
}





% misc

@misc{radford2019gpt2,
  title={Language models are unsupervised multitask learners},
  author={Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
  note={Unpublished manuscript},
  url = {https://d4mucfpksywv.cloudfront.net/better-language-models/language_models_are_unsupervised_multitask_learners.pdf},
  year={2019}
}

@article{Holtzman2019TheCC,
  title={The Curious Case of Neural Text Degeneration},
  author={Ari Holtzman and Jan Buys and Maxwell Forbes and Yejin Choi},
  journal={ICLR},
  year={2020},
}


@article{mikolov2013efficient,
  title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}


@misc{Gokaslan2019OpenWeb,  
	title={OpenWebText Corpus},
	author={Aaron Gokaslan and Vanya Cohen},
	url ="http://Skylion007.github.io/OpenWebTextCorpus", 
	year={2019}
}
@inproceedings{Mao2019PollyWA,
  title={Polly Want a Cracker: Analyzing Performance of Parroting on Paraphrase Generation Datasets},
  author={Hongren Mao and Hungyi Lee},
  booktitle={EMNLP/IJCNLP},
  year={2019}
}

@inproceedings{federmann-etal-2019-multilingual,
    title = "Multilingual Whispers: Generating Paraphrases with Translation",
    author = "Federmann, Christian  and
      Elachqar, Oussama  and
      Quirk, Chris",
    booktitle = "Proceedings of the 5th Workshop on Noisy User-generated Text (W-NUT 2019)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D19-5503",
    doi = "10.18653/v1/D19-5503",
    pages = "17--26",
}


@inproceedings{sun-zhou-2012-ibleu,
    title = "Joint Learning of a Dual {SMT} System for Paraphrase Generation",
    author = "Sun, Hong  and
      Zhou, Ming",
    booktitle = "Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    month = jul,
    year = "2012",
    address = "Jeju Island, Korea",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P12-2008",
    pages = "38--42",
}

@inproceedings{wieting-gimpel-2018-paranmt,
    title = "{P}ara{NMT}-50{M}: Pushing the Limits of Paraphrastic Sentence Embeddings with Millions of Machine Translations",
    author = "Wieting, John  and
      Gimpel, Kevin",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P18-1042",
    doi = "10.18653/v1/P18-1042",
    pages = "451--462"
}

@inproceedings{lin2001dirt,
  title={Dirt@ sbt@ discovery of inference rules from text},
  author={Lin, Dekang and Pantel, Patrick},
  booktitle={Proceedings of the seventh ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={323--328},
  year={2001}
}


@article{radford2018improving,
  title={Improving language understanding by generative pre-training},
  author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya}
}

@inproceedings{kajiwara2019negative,
  title={Negative Lexically Constrained Decoding for Paraphrase Generation},
  author={Kajiwara, Tomoyuki},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={6047--6052},
  year={2019}
}

@article{hinton2002training,
  title={Training products of experts by minimizing contrastive divergence},
  author={Hinton, Geoffrey E},
  journal={Neural computation},
  volume={14},
  number={8},
  pages={1771--1800},
  year={2002},
  publisher={MIT Press}
}

@inproceedings{zellers2019defending,
  title={Defending against neural fake news},
  author={Zellers, Rowan and Holtzman, Ari and Rashkin, Hannah and Bisk, Yonatan and Farhadi, Ali and Roesner, Franziska and Choi, Yejin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={9051--9062},
  year={2019}
}

@inproceedings{wieting2018paranmt,
  title={ParaNMT-50M: Pushing the Limits of Paraphrastic Sentence Embeddings with Millions of Machine Translations},
  author={Wieting, John and Gimpel, Kevin},
  booktitle={Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={451--462},
  year={2018}
}

@inproceedings{bosselut2019comet,
  title={COMET: Commonsense Transformers for Automatic Knowledge Graph Construction},
  author={Bosselut, Antoine and Rashkin, Hannah and Sap, Maarten and Malaviya, Chaitanya and Celikyilmaz, Asli and Choi, Yejin},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={4762--4779},
  year={2019}
}

@inproceedings{bottlesum,
  title={BottleSum: Unsupervised and Self-supervised Sentence Summarization using the Information Bottleneck Principle},
  author={West, Peter and Holtzman, Ari and Buys, Jan and Choi, Yejin},
  booktitle={Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)},
  pages={3743--3752},
  year={2019}
}

@article{shwartz2020unsupervised,
  title={Unsupervised Commonsense Question Answering with Self-Talk},
  author={Shwartz, Vered and West, Peter and Bras, Ronan Le and Bhagavatula, Chandra and Choi, Yejin},
  journal={arXiv preprint arXiv:2004.05483},
  year={2020}
}


@inproceedings{wang-etal-2019-make,
    title = "Does it Make Sense? And Why? A Pilot Study for Sense Making and Explanation",
    author = "Wang, Cunxiang  and
      Liang, Shuailong  and
      Zhang, Yue  and
      Li, Xiaonan  and
      Gao, Tian",
    booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P19-1393",
    doi = "10.18653/v1/P19-1393",
    pages = "4020--4026",
}

@inproceedings{WMT2019,
  title={Findings of the 2019 conference on machine translation (wmt19)},
  author={Barrault, Lo{\"\i}c and Bojar, Ond{\v{r}}ej and Costa-Juss{\`a}, Marta R and Federmann, Christian and Fishel, Mark and Graham, Yvette and Haddow, Barry and Huck, Matthias and Koehn, Philipp and Malmasi, Shervin and others},
  booktitle={Proceedings of the Fourth Conference on Machine Translation (Volume 2: Shared Task Papers, Day 1)},
  pages={1--61},
  year={2019},
  url       = {http://www.aclweb.org/anthology/W19-5301}
}

@misc{martins2020sparse,
    title={Sparse Text Generation},
    author={Pedro Henrique Martins and Zita Marinho and André F. T. Martins},
    year={2020},
    eprint={2004.02644},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}

@article{welleck2019neural,
  title={Neural text generation with unlikelihood training},
  author={Welleck, Sean and Kulikov, Ilia and Roller, Stephen and Dinan, Emily and Cho, Kyunghyun and Weston, Jason},
  journal={arXiv preprint arXiv:1908.04319},
  year={2019}
}


@article{gpt3,
  title={Language models are few-shot learners},
  author={Brown, Tom B and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={arXiv preprint arXiv:2005.14165},
  year={2020}
}

%SARI
@article{xu-etal-2016-optimizing,
    title = "Optimizing Statistical Machine Translation for Text Simplification",
    author = "Xu, Wei  and
      Napoles, Courtney  and
      Pavlick, Ellie  and
      Chen, Quanze  and
      Callison-Burch, Chris",
    journal = "Transactions of the Association for Computational Linguistics",
    volume = "4",
    year = "2016",
    url = "https://www.aclweb.org/anthology/Q16-1029",
    doi = "10.1162/tacl_a_00107",
    pages = "401--415",
    abstract = "Most recent sentence simplification systems use basic machine translation models to learn lexical and syntactic paraphrases from a manually simplified parallel corpus. These methods are limited by the quality and quantity of manually simplified corpora, which are expensive to build. In this paper, we conduct an in-depth adaptation of statistical machine translation to perform text simplification, taking advantage of large-scale paraphrases learned from bilingual texts and a small amount of manual simplifications with multiple references. Our work is the first to design automatic metrics that are effective for tuning and evaluating simplification systems, which will facilitate iterative development for this task.",
}

@inproceedings{chen-dolan-2011-collecting,
    title = "Collecting Highly Parallel Data for Paraphrase Evaluation",
    author = "Chen, David  and
      Dolan, William",
    booktitle = "Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies",
    month = jun,
    year = "2011",
    address = "Portland, Oregon, USA",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P11-1020",
    pages = "190--200",
}


@article{Zhang2020BERTScoreET,
  title={BERTScore: Evaluating Text Generation with BERT},
  author={Tianyi Zhang and V. Kishore and Felix Wu and Kilian Q. Weinberger and Yoav Artzi},
  journal={ArXiv},
  year={2020},
  volume={abs/1904.09675}
}

@inproceedings{Sellam2020BLEURTLR,
  title={BLEURT: Learning Robust Metrics for Text Generation},
  author={Thibault Sellam and Dipanjan Das and Ankur P. Parikh},
  booktitle={ACL},
  year={2020}
}

@article{landis1977measurement,
  title={The measurement of observer agreement for categorical data},
  author={Landis, J Richard and Koch, Gary G},
  journal={biometrics},
  pages={159--174},
  year={1977},
  publisher={JSTOR}
}

@article{fleiss1971measuring,
  title={Measuring nominal scale agreement among many raters.},
  author={Fleiss, Joseph L},
  journal={Psychological bulletin},
  volume={76},
  number={5},
  pages={378},
  year={1971},
  publisher={American Psychological Association}
}

@article{combine_irr,
  title={Nominal scale agreement among observers},
  author={Schouten, Hubert JA},
  journal={Psychometrika},
  volume={51},
  number={3},
  pages={453--466},
  year={1986},
  publisher={Springer}
}

@inproceedings{lan2017continuously,
  author     = {Lan, Wuwei and Qiu, Siyu and He, Hua and Xu, Wei},
  title      = {A Continuously Growing Dataset of Sentential Paraphrases},
  booktitle  = {Proceedings of The 2017 Conference on Empirical Methods on Natural Language Processing (EMNLP)},
  year       = {2017},
  publisher  = {Association for Computational Linguistics},
  pages      = {1235--1245},
  location   = {Copenhagen, Denmark},
  url        = {http://aclweb.org/anthology/D17-1127}
} 

@inproceedings{ma2018results,
  title={Results of the WMT18 metrics shared task: Both characters and embeddings achieve good performance},
  author={Ma, Qingsong and Bojar, Ond{\v{r}}ej and Graham, Yvette},
  booktitle={Proceedings of the third conference on machine translation: shared task papers},
  pages={671--688},
  year={2018}
}

@inproceedings{liu2010pem,
  title={PEM: A paraphrase evaluation metric exploiting parallel texts},
  author={Liu, Chang and Dahlmeier, Daniel and Ng, Hwee Tou},
  booktitle={Proceedings of the 2010 Conference on Empirical Methods in Natural Language Processing},
  pages={923--932},
  year={2010}
}

@article{kendall1938new,
  title={A new measure of rank correlation},
  author={Kendall, Maurice G},
  journal={Biometrika},
  volume={30},
  number={1/2},
  pages={81--93},
  year={1938},
  publisher={JSTOR}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{Brown2020LanguageMA,
  title={Language Models are Few-Shot Learners},
  author={T. Brown and B. Mann and Nick Ryder and Melanie Subbiah and J. Kaplan and Prafulla Dhariwal and Arvind Neelakantan and Pranav Shyam and Girish Sastry and Amanda Askell and Sandhini Agarwal and Ariel Herbert-Voss and G. Kr{\"u}ger and T. Henighan and R. Child and Aditya Ramesh and D. Ziegler and Jeffrey Wu and Clemens Winter and Christopher Hesse and Mark Chen and E. Sigler and Mateusz Litwin and Scott Gray and Benjamin Chess and J. Clark and Christopher Berner and Sam McCandlish and A. Radford and Ilya Sutskever and Dario Amodei},
  journal={ArXiv},
  year={2020},
  volume={abs/2005.14165}
}

@article{Li2021PrefixTuningOC,
  title={Prefix-Tuning: Optimizing Continuous Prompts for Generation},
  author={Xiang Lisa Li and P. Liang},
  journal={ArXiv},
  year={2021},
  volume={abs/2101.00190}
}

@inproceedings{liu2020unsupervised,
  title={Unsupervised Paraphrasing by Simulated Annealing},
  author={Liu, Xianggen and Mou, Lili and Meng, Fandong and Zhou, Hao and Zhou, Jie and Song, Sen},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={302--312},
  year={2020}
}

==> figs/algorithm.tex <==
% % Algorithm
\begin{algorithm}[!t]
\small
\centering
\caption{\scriptsize \method for Paraphrasing}
\label{alg:paraphrasing}
\begin{algorithmic}[1]
\REQUIRE L2R LM estimating $P_{c_{lh}|s}$ and $P_{gen}^{lh}$ \\ \hspace{1.2em} R2L LM estimating $P_{c_{rh}|s}$ and $P_{gen}^{rh}$ \\ \hspace{1.2em} Source text: $s$

$\ $
\SetAlgoLined

\SetKwProg{Def}{function}{:}{}
\Def{\textnormal{sample} ($P_{c|s}$, $P_{gen}$)}
\noindent{$1_{\text{f}}$:\quad  Sample contexts, $c^0...c^{n_{c}} \sim P_{c|s}$\\}
\noindent{$2_{\text{f}}$:\quad learn $\mathbf{w_{c|s}}$ = $\arg\max_{\mathbf{w_{c|s}}} P_{gen}(s)$ \\\qquad $\sum w_{c|s} = 1, w_{c|s}\geq0$}\\
\noindent {$3_{\text{f}}$:\quad prune $w_{c|s}  \notin \text{top}_k(\mathbf{w_{c|s}})$}\\
\noindent {$4_{\text{f}}$:\quad normalize $\mathbf{w_{c|s}} = 
\frac{\mathbf{w_{c|s}}}{\sum w_{c|s}}$}\\
\noindent {$5_{\text{f}}$:\quad Sample generations $\hat{s}^0... \hat{s}^{n_{\hat{s}}} \sim P_{gen}$}\\
\noindent{$6_{\text{f}}$:\quad \textbf{return} $\hat{s}^0... \hat{s}^{n_{\hat{s}}}$}

$\ $


{\color{gray}// Sample with lh contexts}
\STATE $\hat{s}_{lh}^0... \hat{s}_{lh}^{n_{\hat{s}}} \leftarrow$ sample($P_{c_{lh}|s}$, $P_{gen}^{lh}$)\\
{\color{gray}// Sample with rh contexts}
\STATE $\hat{s}_{rh}^0... \hat{s}_{rh}^{n_{\hat{s}}} \leftarrow$ sample($P_{c_{rh}|s}$, $P_{gen}^{rh}$)\\
{\color{gray}// Combine and rank}
\STATE $\mathbf{candidates} = \hat{s}_{lh}^0 ...\hat{s}_{lh}^{n_{\hat{s}}},\hat{s}_{rh}^0 ...\hat{s}_{rh}^{n_{\hat{s}}}$
\STATE TRIM candidates to be proper sentences
\STATE FILTER candidates with bad formatting
\STATE Rank $\mathbf{candidates}$ by $S_p(\hat{s})$
\ENSURE Highest-ranked paraphrase $\hat{s}$
\end{algorithmic}
\end{algorithm}


==> figs/algorithm_anlg.tex <==



% % Algorithm
\begin{algorithm}[!t]
\small
\centering
\caption{\scriptsize \method for $\alpha$NLG}
\label{alg:anlg}
\begin{algorithmic}[1]
\REQUIRE L2R LM estimating $P_{c_{rh}|o_1,o_2}$ and $P_{gen}^{rh}$ \\ \hspace{1.2em} R2L LM estimating $P_{c_{lh}|o_1,o_2}$ and $P_{gen}^{lh}$ \\ \hspace{1.2em} Observations $o_1$ and $o_2$, concatenated as $o_1,o_2$\\
$\ $

\SetAlgoLined

\SetKwProg{Def}{function}{:}{}
\Def{\textnormal{sample} ($P_{c|o_1,o_2}$, $P_{gen}$, \textnormal{dir})}
\noindent{$1_{\text{f}}$:\quad  Sample contexts, $c^0...c^{n_{c}} \sim P_{c|o_1,o_2}$\\}
\noindent{$2_{\text{f}}$:\quad learn $\mathbf{w_{c|o_1,o_2}}$ = $\arg\max_{\mathbf{w_{c|s}}} P_{gen}(o_1,o_2)$ \\\qquad $\sum w_{c|o_1,o_2} = 1, w_{c|o_1,o_2}\geq0$}\\
\noindent {$3_{\text{f}}$:\quad prune $w_{c|o_1,o_2}  \notin \text{top}_k(\mathbf{w_{c|o_1,o_2}})$}\\
\noindent {$4_{\text{f}}$:\quad normalize $\mathbf{w_{c|o_1,o_2}} = 
\frac{\mathbf{w_{c|o_1,o_2}}}{\sum w_{c|o_1,o_2}}$}\\
\noindent {$5_{\text{f}}$:\quad IF dir == $lh$ THEN $c^i = c^i + o_1$ }\\
\noindent {$6_{\text{f}}$:\quad IF dir == $rh$ THEN $c^i = o_2 + c^i$ }\\
\noindent {$7_{\text{f}}$:\quad Sample generations $h^0...h^{n_h} \sim P_{gen}(h)$}\\
\noindent{$8_{\text{f}}$:\quad \textbf{return} $h^0...h^{n_h}$}

$\ $


{\color{gray}// Sample with lh contexts}
\STATE $h_{lh}^0 ...h_{lh}^{n_{h}} \leftarrow$ sample($P_{c_{lh}|s}$, $P_{gen}^{lh}$, lh)\\
{\color{gray}// Sample with rh contexts}
\STATE $h_{rh}^0 ...h_{rh}^{n_{h}} \leftarrow$ sample($P_{c_{rh}|s}$, $P_{gen}^{rh}$, rh)\\
{\color{gray}// Combine and rank}
\STATE $\mathbf{candidates} = h_{lh}^0 ...h_{lh}^{n_{h}},h_{rh}^0 ...h_{rh}^{n_{h}}$
\STATE TRIM candidates to be proper sentences
\STATE FILTER candidates with bad formatting
\STATE Rank $\mathbf{candidates}$ by $P_{L2R}(o_2|o_1 + h)*P_{R2L}(o_1| h + o_2)$
\ENSURE Highest-ranked hypothesis $h$
\end{algorithmic}
\end{algorithm}







==> figs/anlg_results_wrap.tex <==
\begin{wraptable}{r}{7.8cm}
    
    \begin{tabular}{l|ccc|c}
     \toprule
       & $o_1$ & $o_2$ & $o_1+o_2$ & all\\ 
       
    \midrule  
    human & 86.7 & 84.3 & 78.0 & 83.8 \\
   \midrule
   \rowcolor[gray]{0.95} \multicolumn{5}{l}{\textit{Supervised}} \\
   \midrule
   $\text{COMeT}_{\text{Emb}}$+GPT2 & 72.4 & \textbf{61.9} & 55.1 & 60.1 \\ 
   $\text{COMeT}_{\text{Txt}}$+GPT2 & 72.1 & 60.3 & 54.6 & 59.4 \\ 
   $O_1$-$O_2$-Only & \textbf{72.5} & 61.6 & \textbf{55.7} & \textbf{60.9}  \\ 
    \midrule
   \rowcolor[gray]{0.95} \multicolumn{5}{l}{\textit{Unsupervised}} \\
   \midrule
   GPT2-Fixed & 24.2 & 21.0 & 18.5 & 19.3 \\ 
   Reflect Decoding & \textbf{56.7} & \textbf{55.3} & \textbf{46.2} & \textbf{50.0} \\



     \bottomrule
    \end{tabular}
    \caption{Model performance on $\alpha$NLG. The first 3 scores query agreement between hypothesis and given observation(s), and ``all'' indicates overall judgement.}  
    \label{tab:anlg}
\end{wraptable}

==> figs/backups/algorithm_lr_0.tex <==
% % Algorithm

\begin{algorithm}[!t]
\small
\centering
\caption{\scriptsize Learn \decoder (left-to-right)}
\label{alg_lr}
\begin{algorithmic}[1]
\REQUIRE Left to right language model \lrLM \\
\hspace{1.2em} Right to left language model \rlLM \\
 \hspace{1.2em} Source text: $s_{src}$

$\ $
\SetAlgoLined




\STATE  Sample contexts, $c_1...c_{n_{c}} \sim \text{\rlLM}(c|s_{src})$\\\
\STATE Initialize parameters $\mathbf{w} = w_1...w_{n_{c}}$ s.t. $\sum w_i = 1, w_i\geq0$\\\
\STATE learn $\mathbf{w}$ = $\arg\max_{\mathbf{w}} \text{\lrRD}(s_{src})$ \\\qquad under $\sum w_i = 1, w_i\geq0$\\\
\ENSURE $\text{\lrRD}$
\end{algorithmic}
\end{algorithm}


==> figs/backups/anlg_results_0.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccc|c}
     \toprule
       & $o_1$ & $o_2$ & $o_1+o_2$ & all\\ 
       
    \midrule  
    Human & 86.7 & 84.3 & 78.0 & 83.8 \\
   \midrule
   \rowcolor[gray]{0.95} \multicolumn{5}{l}{\textit{Supervised}} \\
   \midrule
   $\text{COMeT}_{\text{Emb}}$+GPT2 & 72.4 & \textbf{61.9} & 55.1 & 60.1 \\ 
   $\text{COMeT}_{\text{Txt}}$+GPT2 & 72.1 & 60.3 & 54.6 & 59.4 \\ 
   $O_1$-$O_2$-Only & \textbf{72.5} & 61.6 & \textbf{55.7} & \textbf{60.9}  \\ 
    \midrule
   \rowcolor[gray]{0.95} \multicolumn{5}{l}{\textit{Unsupervised}} \\
   \midrule
   GPT2-Fixed & 24.2 & 21.0 & 18.5 & 19.3 \\ 
   Reflective Decoding & \textbf{56.7} & \textbf{55.3} & \textbf{46.2} & \textbf{50.0} \\



     \bottomrule
    \end{tabular}
    \caption{Model performance on $\alpha$NLG. The first 3 scores query agreement between hypothesis and given observation(s), ``all'' indicates overall judgement. \method significantly outperforms the unsupervised baseline.}  
    \label{tab:anlg}
\end{table}

==> figs/backups/model_params_0.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cc}
     \toprule

      Param & Paraphrasing & $\alpha$NLG\\ 
 \midrule
   model size & Mega & Mega \\
%   $lh$ & `` & O1 \\ 
%   $rh$ & '' & O2 \\ 
%   $s_{mid}$ & $s$ & empty \\ 
   $len_{\hat{s}}\text{ or } len_{h}$ & len$(s)+5$ & 20 \\ 
   $len_c$ & 50 & 50 \\ 
   $n_{\hat{s}}$ & 30 & 20 \\
   $n_{c}$ & 80 & 50 \\
   $h_{sample}$ & 4. & 6. \\
   $p_{c}$ & 0.7 & 0.9 \\
   $k_c$ & 6 & 6 \\
    \bottomrule
    \end{tabular}
    \caption{Most parameters are explained in  \S\ref{subsec:implementation}. $h_{sample}$ is entropy for sampling calibration in \S\ref{app:entropy_calibtration} } % 
    \label{tab:params}
\end{table}

==> figs/backups/twitter_results_0.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{ll|cccc|c}
     \toprule
 & Method & SARI$\uparrow$ & BLEU$\uparrow$ & METEOR$\uparrow$ & TER$_{P}$$\downarrow$ &  $Novelty\uparrow$ \\ 
 \midrule
 \textit{Human} & Source & 13.6 & 36.7 & 25.0 & 75.0 & 0.0 \\
   & Reference & 90.7 & 100.0 & 100.0 & 0.0 & 63.3 \\ 
 \midrule
   \textit{Supervised (Bilingual)} & MT & 36.1 & 29.4 & 22.1 & 80.0 & 30.4\\
   \midrule
  \textit{Unsupervised} & R-VQVAE & 31.1 & 25.2 & 21.0 & 90.0 & 40.4\\ 
   & CGMH$_{Top}$&  32.7 & 28.2 & 19.8 & 77.0 & 25.5\\
   & CGMH$_{30}$&  33.2 & 26.3 & 18.7 & 78.0 & 30.1\\
   & CGMH$_{45}$&  31.8 & 20.5 & 15.4 & 82.0 & 45.7\\
  & RD$_{Top/30}$ (Us) & 31.4 & 27.2 & 19.9 & 86.0 & 37.0\\
   & RD$_{45}$ (Us) & 36.1 & 25.6 & 19.0 & 88.0 & 45.3\\
    \bottomrule
    \end{tabular}
    \caption{Model performance on the Twitter URL test split. \textbf{Bold} indicates best for model-type, * indicates best overall (excluding human). The first 4 columns are measures of quality, while the last measures novelty (equation \ref{eqn:novelty}) or dissimilarity from input. We rerun evaluations from past work. Note: Diversity of RD$_{Top}$ is over 30 and so this model is equivalent to RD$_{30}$ here.}
    
    \label{tab:twitter_results}
\end{table*}

==> figs/diversity_v_quality.tex <==
\begin{figure*}[t]
    \centering

    \includegraphics[width=1.0\linewidth]{figs/diversity_v_quality.png}
    
    \caption{Plotting notions of quality against diversity from Table~\ref{tab:quoratest}. We plot across a wider range of diversity cutoffs for Reflective Decoding (us) and CGMH on automatic metrics. Table \ref{tab:quoratest} has a subset of the diversities here.}
    \label{diversit_v_quality}
\end{figure*} 

==> figs/gen_examples_1.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=0.87\linewidth]{figs/table_1_v3.pdf}
     \caption{\method generations. Quora aims to paraphrase, and $\alpha$NLG aims to fill in the blank. For Quora, RefDec-50 forces more diversity from the source sentence than RefDec-70.} 
\end{figure*} 

==> figs/gen_examples_2.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=1.0\linewidth]{figs/page-wide_v5.pdf}
    \caption{Generation examples for $\alpha$NLG and paraphrasing from all tested systems}  % 
    \label{fig_gen_examples_2}
\end{figure*} 

==> figs/novelty_v_quality.tex <==
\definecolor{mypink1}{rgb}{1., 0.5, 0.5}

\definecolor{myblue}{rgb}{0.5, 0.5, 0.8}

\definecolor{mygreen}{rgb}{0.5, 0.8, 0.5}

%\begin{wrapfigure}{r}{0.5\linewidth}
\begin{figure}
%\begin{figure*}[t]
    \centering

    \includegraphics[width=0.8\textwidth]{figs/novelty_v_quality.png}
    
    \caption{Plotting notions of quality against novelty from Table~\ref{tab:quoratest}, by color: \method in \textbf{BLACK}, unsupervised baselines in  \textcolor{mypink1}{\textbf{RED}}, MT in \textcolor{myblue}{\textbf{BLUE}}, and supervised in \textcolor{mygreen}{\textbf{GREEN}}. Using plot a range of Novelty cutoffs for \method and CGMH.}
    \label{diversit_v_quality}
\end{figure} 

%\end{wrapfigure}

==> sections/backups/introduction_0.tex <==
\section{Introduction}
\label{introduction}


%\input{figs/gen_examples_1}
%\input{figs/gen_examples_2}

%\input{figs/generations_1}





Pretrained language models (LMs) have made remarkable progress in language generation. % -- a critical aspect of human intelligence.
% Language generation is a central aspect of human intelligence, which large pretrained language models (LMs) have recently propelled machines towards.
Trained over large amounts of unstructured text, models like GPT2 \citep{radford2019gpt2} leverage enhanced generation methods  \citep{Holtzman2019TheCC, martins2020sparse, welleck2019neural} resulting in fluent and coherent continuations to given input text—e.g. news articles or stories. 

\input{figs/fig_1}

%\ari{However, it’s unclear how to apply LMs to tasks that cannot be framed as left-to-right generation—e.g.  paraphrasing and text-infilling. Still, LMs undeniably model notions of “semantic neighborhood” and “contextual fit” inherent in these tasks: to predict what sentence comes next, a model must implicitly capture a subspace of similar sentences that fit the context.  Can we leverage this inherent knowledge of LMs and apply them to these tasks without direct supervision?}
%\cs{Possible rewrite of this paragraph: However, LMs cannot be applied directly to tasks that cannot be framed as left-to-right generation -- e.g. paraphrasing and text-infilling. They need to be finetuned specifically for such tasks with task-specific supervision. We hypothesize that LMs inherently capture the semantics required to solve these tasks, but they are restricted by their left-to-right nature. \textit{Can we leverage this inherent knowledge of LMs and apply them to these tasks without direct supervision?}}
However, it’s unclear how to apply LMs to tasks that cannot be framed as left-to-right generation—e.g.  paraphrasing and text infilling—without additional task-specific supervision. Yet, LMs implicitly model the notions of “semantic neighborhood” and “contextual fit” inherent in these tasks: to predict the next sentence, a model must implicitly capture a subspace of similar sentences related to the given context. We leverage this latent knowledge to apply pretrained LMs to non-sequential tasks without direct supervision.

%\peter{original: Yet there seems to be a gap for LMs between potential and practice. Pretrained LMs do not readily solve tasks like paraphrasing and text-infilling, which cannot easily be framed as left-to-right continuation. Still, LMs undeniably model notions of ``semantic neighborhood'' and ``contextual fit'' inherent in these tasks: to predict what sentence comes next, a model must implicitly capture a subspace of similar sentences that fit the context. How can we access this knowledge? }

 
%\cs{Possible rewrite: We introduce \method{} -- a novel decoding method that allows LMs to be applied to paraphrasing and text-infilling, without task-specific supervision. \method{} relies on the availability of two complementary LMs -- one forward (\lrLM) and a backward (\rlLM). \lrLM{} (resp., \rlLM) is trained to generate text left-to-right (resp., right-to-left). }
We introduce  \method—a novel decoding method that allows LMs to be applied to naturally distributional tasks like paraphrasing and text-infilling. \method{} requires \textit{no} supervision, only two complementary LMs—one forward (\lrLM) and one backward (\rlLM) trained to generate text left-to-right and right-to-left (respectively). 
%\ari{Changed this a bit and now I think it's the best of both worlds :)}
%\yejin{i like these notations! but the way they are introduced can be easily ignored. i.e., readers might not associate which is forward and which is backward right away. i think it's better if we make this really explicit}



%\cs{Possible rewrite: Inspired by the distributional hypothesis for representing the \textit{meaning} of words using other words in its context \cite{}, the two LMs are used to generate \textit{contexts} that can represent the \textit{meaning} of a given sentence. First, in the \stepone{}, the forward LM (\lrLM) is used to generate multiple sentences that can \textit{follow} the input sentence, $s_{src}$. We refer to this set of generated sentences as the \textit{right-handed context}. Similarly, the backward LM (\lrLM) is used to generate \textit{left-handed context}. Next, in the \steptwo, the left-handed context (resp., right-handed context) is used as input to decode its meaning using its converse LM -- i.e. \lrLM{} (resp., \rlLM).}

Inspired by the distributional hypothesis 
%for representing the meaning of a word using other words it often co-occurs with 
\citep{firth1957synopsis}, we use two LMs to generate \textit{contexts} that collectively represent the meaning of a given input, by constraining what could occur between ensembles of these left- and right-hand contexts (the \stepone). In the \steptwo we decode with this meaning representation by conditioning on an ensemble of these contexts from either side, generating contextually similar outputs.%, then scoring them by considering both left- and right-hand ensembles together.
%We then \textit{learn} a sampling function that generates by ensembling the distribution imposed by the generated contexts. % \ari{I think this explanation is a bit confusing...right not it reads as trying to slide over the details but possibly further confusing the reader as to what kind of learning is going on and when.}

%\cs{Figure \ref{fig_1} (left) shows an example of \method applied to paraphrasing. Given an input $s_{src}:$ \textit{How are circulatory system tissues formed?}, the \stepone generates contexts $c_i$ for $s_{src}$ with a language model \lrLM. Each context captures different aspect of the input sentence -- e.g. $c_1$: \textit{This is a medical question} situates the input as a question, and $c_2$: \textit{As with all tissue in the body...} presents an elaboration of the central concept in $s_{src}$. Collectively, they capture the meaning of the input sentence. Next, we sample outputs in the \steptwo. Weighting the generated contexts with a backwards language model (\rlLM), we learn a sampling function that \textit{reflects} back from the \textit{context} to generate a sentence with the same meaning as the input text.}
% gazebo
Figure \ref{fig_1} (top) shows an example of \method applied to paraphrasing, with the left-side contexts omitted for clarity. Given an input $s_{src}:$ \textit{How are circulatory system tissues formed?} the \stepone generates contexts $c_i$ for $s_{src}$ with \lrLM, each capturing different aspects of the input sentence -- e.g. $c_1$: \textit{This is a medical question} situates the input as a question, and $c_2$: \textit{As with all tissue in the body...} presents an elaboration of the central concept in $s_{src}$ (tissue formation). Collectively, many contexts capture the meaning of the input sentence. Next, we sample outputs in the \steptwo. By conditioning on the generated contexts with a backwards language model (\rlLM) in a weighted ensemble \rlRD, we \textit{reflect} back from the contexts to generate a sentence with the same meaning as the input text.
% My old version
%The left side of Figure \ref{fig_1} sheds light on how this proceeds for paraphrasing. Given an input $s_{src}:$ \textit{How are circulatory system tissues formed?} we start with the \stepone, generating contexts $c_i$ for $s_{src}$ with a language model \lrLM. Some of these situate the sentence as a question ($c_1$: \textit{This is a medical question}), while others elaborate on the central concept ($c_1$: \textit{As with all tissue in the body...}). Over many contexts we capture the full meaning. Next, we sample outputs in the \steptwo. Weighting these contexts with a language model \rlLM in the opposite direction, we learn a sampling function that \textit{reflects} back from the \textit{context} to the \textit{text} with the original meaning. In paraphrasing, we use this to repeat the meaning of the source; in text infilling, it allows us to consider information from two-sided context.  

\method shows strong unsupervised performance: On the Quora paraphrasing dataset, we test with multiple levels of $Novelty$ (variation from the source sentence) finding one setting ($\text{RD}_{30}$) outperforms unsupervised baselines on all but one metric, and supervised baselines on both the SARI metric and human evaluation. %\cs{Replace next sentence: We also apply \method{} to $\alpha$NLG (\cite{Bhagavatula2019AbductiveCR})--a text-infilling task--and show that it outperforms the unsupervised baseline on overall quality by 30.7 points, and significantly closes the gap with supervised methods.} 
%In $\alpha$NLG we outperform the unsupervised baseline on overall quality by 30.7 points, and significantly close the gap with supervised methods. 
Applying \method{} to $\alpha$NLG \citep{Bhagavatula2019AbductiveCR}---a text infilling task---we outperform the unsupervised baseline on overall quality by 30.7 points, significantly closing the gap with supervised methods. In both applications, \method proceeds without any finetuning, directly using pretrained models. 

Our results suggest that completely unsupervised generation can solve a number of tasks with thoughtful decoding choices, analogous to GPT-3 \citep{gpt3} showing the same for thoughtfully designed contexts. These are supported by extensive further experiments in the appendix, and an intuitive interpretation of \method{} in \S\ref{subseq_intuitions_and_theory}: sampling while restricting contextual (i.e. distributional) similarity with respect to the source text. \method{} is an exciting example of how far unsupervised learning can take us, when we design methods for eliciting specific kinds of information from pretrained LMs. % \ari{This is good, but probably a little too "woo" for most NLP researchers. Let's keep it, but engineer it to be just a smidgeon more presentable.}
%\ari{This part is pretty good, but still reads a little milquetoast without the right emphasis on how little supervision we're working with till the end.} %\peter{Keeping this in as a reminder I need to highlight this}

%\ari{describe extensiveness}

==> sections/backups/introduction_1.tex <==
\section{Introduction}
\label{introduction}


%\input{figs/gen_examples_1}
%\input{figs/gen_examples_2}

%\input{figs/generations_1}

% Pretrained language models (LMs) have made remarkable progress in language generation. 
Models like GPT-2 \citep{radford2019gpt2}, trained over vast unstructured data, can leverage enhanced generation methods \citep{Holtzman2019TheCC, martins2020sparse, welleck2019neural} to give fluent and coherent continuations to given input text—e.g. news articles or stories. GPT-3 \citep{Brown2020LanguageMA} takes this a step further: given a small number of examples and a well-constructed prompt, it shows remarkable performance on tasks where supervision was thought to be necessary, no tuning required. While this demonstrates the potential for Language Models in  few-shot or even zero-shot out-of-the-box settings, limited access to GPT-3 and immense computational cost keep this from being a widely usable or efficient solution. % Peter: Besides being inaccessible/expensive, applying GPT3 this way demands a model both know how to do a task, and understand, from a prompt (e.g. paraphrase this sentence) that this is what is being asked of it. There is significant room in the middle, for models which are capable of task, but must be asked nicely.
\input{figs/fig_1}

Yet recent work shows that GPT-2 may hold similar capabilities. \citet{Li2021PrefixTuningOC} also achieve supervised-level performance in a few-shot setting, but using smaller, accessible models like GPT-2. They learn a small number of task-specific vectors as a prefix to the input, holding the model itself static. Off-the-shelf GPT-2 is capable of few-shot learning given the right cue, in this case taking the form of a small number of input vectors. Our work aims to follow this notion, but beyond few-shot tuning to unsupervised, out-of-the-box decoding.

% Peter - workshopping the first two paragraphs
% Meanwhile, GPT3 \citep{Brown2020LanguageMA} demonstrates the potential for LMs to solve tasks s ... Recent work \cite{Li2021PrefixTuningOC} shows that GPT2 can similarly solve typically supervised tasks (e.g. table-to-text generation) simply by adding input embeddings under limited supervision, leaving the main model parameters static. Like GPT3, the much smaller and more accessible GPT2 seems fundamentally capable of solving complex tasks outside of text continuation. 

%However, it’s unclear how to apply LMs to tasks that cannot be framed as left-to-right generation—e.g.  paraphrasing and text infilling—without additional task-specific supervision. Yet, LMs implicitly model the notions of “semantic neighborhood” and “contextual fit” inherent in these tasks: to predict the next sentence, a model must implicitly capture a subspace of similar sentences related to the given context. We leverage this latent knowledge to apply pretrained LMs to non-sequential tasks without direct supervision.

%\peter{original: Yet there seems to be a gap for LMs between potential and practice. Pretrained LMs do not readily solve tasks like paraphrasing and text-infilling, which cannot easily be framed as left-to-right continuation. Still, LMs undeniably model notions of ``semantic neighborhood'' and ``contextual fit'' inherent in these tasks: to predict what sentence comes next, a model must implicitly capture a subspace of similar sentences that fit the context. How can we access this knowledge? }

 
%\cs{Possible rewrite: We introduce \method{} -- a novel decoding method that allows LMs to be applied to paraphrasing and text-infilling, without task-specific supervision. \method{} relies on the availability of two complementary LMs -- one forward (\lrLM) and a backward (\rlLM). \lrLM{} (resp., \rlLM) is trained to generate text left-to-right (resp., right-to-left). }
We introduce  \method—a novel decoding method that allows LMs to be applied to naturally distributional tasks which break the unidirectional paradigm, like paraphrasing and text-infilling. \method{} requires \textit{no} supervision, only two complementary LMs—one forward (\lrLM) and one backward (\rlLM) trained to generate text left-to-right and right-to-left (respectively). 
%\ari{Changed this a bit and now I think it's the best of both worlds :)}
%\yejin{i like these notations! but the way they are introduced can be easily ignored. i.e., readers might not associate which is forward and which is backward right away. i think it's better if we make this really explicit}



%\cs{Possible rewrite: Inspired by the distributional hypothesis for representing the \textit{meaning} of words using other words in its context \cite{}, the two LMs are used to generate \textit{contexts} that can represent the \textit{meaning} of a given sentence. First, in the \stepone{}, the forward LM (\lrLM) is used to generate multiple sentences that can \textit{follow} the input sentence, $s_{src}$. We refer to this set of generated sentences as the \textit{right-handed context}. Similarly, the backward LM (\lrLM) is used to generate \textit{left-handed context}. Next, in the \steptwo, the left-handed context (resp., right-handed context) is used as input to decode its meaning using its converse LM -- i.e. \lrLM{} (resp., \rlLM).}

Inspired by the distributional hypothesis 
%for representing the meaning of a word using other words it often co-occurs with 
\citep{firth1957synopsis}, \method works by generating text that might occupy the \emph{same contexts} as an input, i.e. replacing it in-context. In practice, we use our two LMs to \textit{generate contexts} that capture aspects of a given input, constraining what might occur between these left- and right-hand contexts (the \stepone). In the \steptwo we decode in the opposite direction--back towards the input--while conditioning on this ensemble of contexts, resulting in generations that are distributionally related to, or replace, the input.%, then scoring them by considering both left- and right-hand ensembles together.
%We then \textit{learn} a sampling function that generates by ensembling the distribution imposed by the generated contexts. % \ari{I think this explanation is a bit confusing...right not it reads as trying to slide over the details but possibly further confusing the reader as to what kind of learning is going on and when.}

%\cs{Figure \ref{fig_1} (left) shows an example of \method applied to paraphrasing. Given an input $s_{src}:$ \textit{How are circulatory system tissues formed?}, the \stepone generates contexts $c_i$ for $s_{src}$ with a language model \lrLM. Each context captures different aspect of the input sentence -- e.g. $c_1$: \textit{This is a medical question} situates the input as a question, and $c_2$: \textit{As with all tissue in the body...} presents an elaboration of the central concept in $s_{src}$. Collectively, they capture the meaning of the input sentence. Next, we sample outputs in the \steptwo. Weighting the generated contexts with a backwards language model (\rlLM), we learn a sampling function that \textit{reflects} back from the \textit{context} to generate a sentence with the same meaning as the input text.}
% gazebo
Figure \ref{fig_1} (top) shows an example of \method applied to paraphrasing, with the left-side contexts omitted for clarity. Given an input $s_{src}:$ \textit{How are circulatory system tissues formed?} the \stepone generates contexts $c_i$ for $s_{src}$ using forward language model \lrLM. Each $c_i$ captures different aspects of the input sentence -- e.g. $c_1$: \textit{This is a medical question} situates the input as a question, and $c_2$: \textit{As with all tissue in the body...} presents an elaboration of the central concept in $s_{src}$ (tissue formation). Collectively, many contexts capture a contextual notion of the input sentence. In the \steptwo, we sample outputs that fit these contexts. By conditioning on the generated contexts with a backwards language model (\rlLM) in a weighted ensemble \rlRD, we \textit{reflect} back from the contexts to generate a sentence with that can replace the input.
% My old version
%The left side of Figure \ref{fig_1} sheds light on how this proceeds for paraphrasing. Given an input $s_{src}:$ \textit{How are circulatory system tissues formed?} we start with the \stepone, generating contexts $c_i$ for $s_{src}$ with a language model \lrLM. Some of these situate the sentence as a question ($c_1$: \textit{This is a medical question}), while others elaborate on the central concept ($c_1$: \textit{As with all tissue in the body...}). Over many contexts we capture the full meaning. Next, we sample outputs in the \steptwo. Weighting these contexts with a language model \rlLM in the opposite direction, we learn a sampling function that \textit{reflects} back from the \textit{context} to the \textit{text} with the original meaning. In paraphrasing, we use this to repeat the meaning of the source; in text infilling, it allows us to consider information from two-sided context.  

Paraphrasing is a natural application, where \method shows strong unsupervised performance: On the Quora dataset, we find one variant of our model ($\text{RD}_{30}$) outperforms unsupervised baselines on all but one metric, and supervised baselines on both the SARI metric and human evaluation. Results on the Twitter dataset support this. %\cs{Replace next sentence: We also apply \method{} to $\alpha$NLG (\cite{Bhagavatula2019AbductiveCR})--a text-infilling task--and show that it outperforms the unsupervised baseline on overall quality by 30.7 points, and significantly closes the gap with supervised methods.} 
%In $\alpha$NLG we outperform the unsupervised baseline on overall quality by 30.7 points, and significantly close the gap with supervised methods. 
By conditioning decoding on part of the input, \method can further be applied to tasks like infilling; applying this to $\alpha$NLG \citep{Bhagavatula2019AbductiveCR}, we outperform the best unsupervised baseline on overall quality by 16.9 points, significantly closing the gap with supervised methods. In both applications, \method proceeds without finetuning, directly using off-the-shelf pretrained models. 
%Our results suggest that completely unsupervised generation can solve a number of tasks with thoughtful decoding choices, analogous to GPT-3 \citep{gpt3} showing the same for thoughtfully designed contexts. These are supported by extensive further experiments in the appendix, and an intuitive interpretation of \method{} in \S\ref{subseq_intuitions_and_theory}: sampling while restricting contextual (i.e. distributional) similarity with respect to the source text.
This is an exciting example of how far unsupervised learning can take us, when we design methods for eliciting specific kinds of information from pretrained LMs. % \ari{This is good, but probably a little too "woo" for most NLP researchers. Let's keep it, but engineer it to be just a smidgeon more presentable.}
%\ari{This part is pretty good, but still reads a little milquetoast without the right emphasis on how little supervision we're working with till the end.} %\peter{Keeping this in as a reminder I need to highlight this}

%\ari{describe extensiveness}

==> sections/backups/methods_0.tex <==
\section{Method}
\label{sec_method}

\subsection{Notation}
\label{subsec_notation}

Arrows indicate the order in which sampling functions condition on and generate tokens: $\xrightarrow{}$ indicates generating from the left-most token to the right (left-to-right), while $\xleftarrow{}$ indicates going right-to-left. For language models (LMs), this means \lrLM is what is often called a ``forward LM'', while \rlLM is a ``backward LM''. For the sampling function (RD), % \lrRD generates tokens left-to-right and \rlRD right-to-left. 
this also indicates which context is being conditioned on, e.g. \lrRD conditions on left context, and extends it to the right to generate output.
% \rlRD conditions on the right context, and generates backward (right-to-left). \lrLM and \rlLM are used together to score candidates, capturing bidirectional context.


\subsection{Overview} 
\label{subseq_overview}

Currently, LM-decoding is limited to a text continuation paradigm. Given an input text $s_{inp}$, $LM(c|s_{inp})$ generates contexts $c$ that might come after (forward) or before (backward) the input. LM-decoding generates \textit{outside} of the input by continuing it, but many tasks require us to generate \textit{within} the input: Paraphrasing requires reformulating the input, while infilling requires adding text in the middle of it. 

Reflective Decoding approaches this shortcoming by turning conventional LM-decoding around: $LM(c|s_{inp})$ generates the kinds of contexts the input might appear in, while $RD(text)$ (defined for $input$) gives the kinds of texts that might also appear in those contexts. In effect, Reflective Decoding generates back \textit{into} the input: $RD(input)$ should be high, the input is likely to appear in its own contexts by definition, but so should texts that might replace $input$ in-context. The distributional hypothesis \citep{firth1957synopsis} suggests semantically similar texts will appear in similar contexts, making paraphrasing an exciting application. 

Concretely, \method breaks out of text-continuation by applying it twice: first in one direction (e.g. forward with \lrLM in Figure \ref{fig_1}) sampling many possible contexts $c_i$ that could follow the input. This is the \textbf{\stepone}. Second, in the \textbf{\steptwo}, we apply a reverse-direction LM (backward \rlLM in Figure \ref{fig_1}) to extend the contexts back, generating text which--like $s_{src}$--fits in these contexts. Assuming contexts $c_i$ are generated in the forward direction, Reflective Decoding takes an intuitive form:

\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{Z(s,c,w) }
    \label{eq:RD_simple}
\end{equation}
\noindent
where the $Z$ function simply normalizes for token-by-token generation (see equation \ref{eqn:rd} ). By taking an ensemble (Product of Experts \citep{hinton2002training}) between the contexts, we can generate $s$ that fits the full set of them. Importantly, weights $w_i$ are learned to prioritize the most informative contexts $c_i$. \peter{we can consider adding the ``weights learned to maximize $s_{src}$ because we \textit{know} it appears here'' intuition with pointers to 2.7, A.1, but maybe we want this somewhere else or nowhere? We should discuss}

The applicability of \method relies on contexts containing expressive information about the input to inform output $s$. To justify how generated contexts might do this, consider the paraphrasing example from Figure~\ref{fig_1} with input $s_{src}:$ \textit{How are circulatory system tissues formed?} Generated contexts reflect different aspects of $s_{src}$: $c_1$ situates $s_{src}$ as a question (\textit{This is a medical question...}), while $c_2$ and $c_3$ explore central concepts  (\textit{as with all tissue...}; \textit{about the circulatory system}). While each context could follow many sentences, together they form a fingerprint for $s_{src}$. A sentence that could be followed by all of $c_1,c_2,c_3$ will likely be a question ($c_1$) about tissue formation ($c_2$) and the circulatory system ($c_3$), and generally occupy the same semantic neighborhood as $s_{src}$: \textit{How do circulatory systems form?}

\peter{Then, last section connecting to infilling and other possible applications. I'm picturing this beginning something like "in paraphrasing, we are replacing all of $s_{src}$ with something that might appear in the same contexts. This is not necessary however, we might replace only part of a sentence (e.g. in context paraphrasing) or even insert text in a gap (text infilling) simply by holding part of $s_{src}$ static when we generate". Not sure if this is the best tactic though, I'm open to anything. }



\peter{JUST doing some brainstorming above, don't mind me
\peter{=============}}

Currently, LM-decoding is constrained to a text-continuation paradigm. Given an input, a forward LM can generate its continuation to the right, and a backward LM its continuation to the left. However, many tasks can't be easily framed this way, e.g. in paraphrasing we want to reword the input, extending it in one direction or the other is insufficient.

% \method extends LM decoding to new tasks—like paraphrasing and infilling—by breaking out of the text-continuation paradigm. 
Rather than extending an input, \method generates outputs that \textit{replace} a span in the input with text that is \textit{similar} to the selected span and \textit{compatible} with the rest. When the span being replaced is the entire input, this corresponds with paraphrasing. When the span being replaced is of length 0, generation is only constrained by context and this corresponds with infilling.


\method operates by generating weighted \textit{context ensembles} that represent the meaning of a span. Paraphrasing is a natural application: distributional intuitions \citep{firth1957synopsis} suggest semantically similar texts appear in similar contexts, so text that fits the same contexts as the input is likely to paraphrase it. $\alpha$NLG \citep{Bhagavatula2019AbductiveCR} is the task of generating a sentence that fits a given left \textit{and} right context, i.e. replacing the 0-length gap inbetween two contexts, and is thus a natural second application.

\method breaks out of text-continuation by applying it twice: first in one direction (e.g., forward with \lrLM in Figure~\ref{fig_1}) sampling many contexts for the input. This is the \textbf{\stepone}. Second, in the \textbf{\steptwo}, these contexts are used with the reverse direction LM (e.g., backward with \rlLM in Figure~\ref{fig_1}) to generate text that fits the ensembled \textit{set} of contexts that were generated.

The applicability of \method relies on contexts containing expressive information about the input. To justify how generated contexts might do this, consider the example from Figure~\ref{fig_1} with input $s_{src}:$ \textit{How are circulatory system tissues formed?} Generated contexts reflect different aspects of $s_{src}$: $c_1$ situates $s_{src}$ as a question (\textit{This is a medical question...}), while $c_2$ and $c_3$ explore central concepts  (\textit{as with all tissue...}; \textit{about the circulatory system}). While each context could follow many sentences, together they form a fingerprint for $s_{src}$. A sentence that could be followed by all of $c_1,c_2,c_3$ will likely be a question ($c_1$) about tissue formation ($c_2$) and the circulatory system ($c_3$), and generally occupy the same semantic neighborhood as $s_{src}$: \textit{How do circulatory systems form?}

Generating a set of contexts is straightforward: we can sample from a pretrained LM (\lrLM above) conditioned on the input $s_{src}$, which captures the distribution of surrounding text. This is the \stepone. To generate back into the input space, we want to sample texts that replace $s_{src}$ and are equally compatible with these generated contexts. To consider all of them when decoding, we condition on an ensemble of contexts in the reverse direction:

\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{Z(s,c,w) }
    \label{eq:RD_simple}
\end{equation}

\noindent
where the $Z$ function simply normalizes for token-by-token generation (see equation \ref{eqn:rd} ). This can be understood as a Product of Experts \citep{hinton2002training} between the contexts.
% preferring generations that \rlLM predicts to precede \textit{all} of the contexts $c_i$. 

Some contexts are more informative than others (i.e. probable but generic contexts like ``See the appendix for details.'' is not very informative), so we weight contexts based on informativeness to $s_{src}$. Weights $w_i$ are learned at inference-time to maximally produce the input $s_{src}$ under equation \ref{eq:RD_simple}. This can be seen as autoencoding, using weighted ensembles of contexts as a meaning representation.
These weights allow us to capture the semantics of $s_{src}$ by capturing how each context \textit{implies} $s_{src}$ as part of the ensemble (see \S\ref{subseq_intuitions_and_theory}, \S\ref{app:derivation}).

In the case of paraphrasing, we would like to replace the entire input. Thus, we simply sample from \rlRD (or the symmetric version, \lrRD from \S\ref{app:lr}), choosing the best output with bidirectional scoring (\S\ref{subsec:app_paraphrase}). 
In $\alpha$NLG the input is sentences $o_1,o_2$ and the task is to generate a third sentence that \textit{bridges} the narrative gap between them. Here, the challenge for LM-decoding is making use of context from both sides ($o_1$ on the left and $o_2$ on the right). \method allows us to generate 1-sided contexts that capture information about both $o_1$ and $o_2$, then replace the 0-length gap between them by appending $o_1$ and $o_2$ to the forward and backward context ensembles, respectively (\S\ref{subsec:app_anlg}). 

\subsection{\method}
\label{subsec:reflective_decoder}

\input{figs/algorithm_simple}


% We proceed to explicitly describe the steps to generate with \method, which requires an input text $s_{src}$, as well as forward and backward language models (\lrLM and \rlLM). From \S\ref{subseq_overview}, 
\method generates outputs that fit the same contexts as the input $s_{src}$, with the option to only overwrite a sub-span of $s_{src}$. By first generating representative contexts, then conditioning a language model in the reverse direction under a weighted ensemble of those contexts (equation \ref{eq:RD_simple}) we define the sampling function (RD), e.g \rlRD in Algorithm~\ref{alg}. For example, consider the right-hand context ensemble, keeping in mind that the process is repeated on the left-hand as well.

First, in the \textbf{\stepone} (line 1), we sample many right-hand contexts $c_i$ for $s_{src}$, using \lrLM. These will be used as a representative sample of the kind of contexts $s_{src}$ appears in.

Second, in the \textbf{\steptwo} (lines 2 - 3) our goal is to sample texts that appear in these same contexts. We construct the sampling function:
\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{ \prod_{j=0}^{|s|} \sum_{t \in V}  \prod_{i}  \text{\rlLM}(t|s_{j+1:|s|} + c_i)^{w_i} }
    \label{eqn:rd}
\end{equation}

\noindent
This is equivalent to equation \ref{eq:RD_simple}, substituting the exact normalization factor for $Z$. Equation~\ref{eqn:rd} is a token-wise Product of Experts model, that captures the semantic neighborhood of $s_{src}$ via the combination of contexts $c_i$ and their weights $w_i$ (\S\ref{subseq_intuitions_and_theory}). 
Our goal is to learn $w_i$ that maximize \rlRD$(s_{src})$, i.e. the probability of generating $s_{src}$. We initialize these weights (line 2),  then train them (line 3) using the Adam optimizer \citep{kingma2014adam}. We normalize weights to be a proper distribution at every step (see \S\ref{app:derivation}). Note, \lrRD is symmetrically learned in the reverse direction, flipping the roles of \lrLM and \rlLM and sampling left-hand context instead (see \S\ref{app:lr} for details).

Finally, we sample from \rlRD (and \lrRD), generating outputs that would appear in the same contexts as $s_{src}$. Depending on the application, we rank and select a final output in different ways. 


\input{figs/fig_examples}



\subsection{Implementation}
\label{subsec:implementation}

% Here, we cover implementation details for \S\ref{subsec:reflective_decoder}.

\paragraph{Weight Learning and Pruning} Weights $w_i$ are learned using the Adam optimizer \citep{kingma2014adam}. In practice this takes under 100 steps (negligible time compared to LM decoding). While we sample tens of contexts (line 1 of Algorithm~\ref{alg}), many end up with negligible weight under the learned distribution (equation \ref{eqn:rd}). To efficiently sample from this function, we drop all but the top $k_c$ contexts and renormalize weights: $k_c < n_c$ contexts are used during the \steptwo.
% described in \S\ref{subsec:reflective_decoder}. 


\paragraph{Parameters} We sample $n_c$ contexts to describe the source $s_{src}$. We use nucleus sampling \citep{Holtzman2019TheCC} with parameter $p_c$, and a maximum length of $len_c$. 
% As stated in \textbf{Weight Pruning}, we drop all but the top $k_c$ contexts by weight.
Once \lrRD and \rlRD are learned, we sample $n_{\hat{s}}$ generations from each, of length $len_{\hat{s}}$. We choose sampling  $p_{\hat{s}}$ per-example to account for vastly different entropy in RD (\S\ref{app:entropy_calibtration}). Values for all hyperparameters are available in \S\ref{app:model_params}.

\paragraph{Language Models} We train large forward (\lrLM) and backward (\rlLM) language models based on GPT2 \citep{radford2019gpt2}  using the OpenWebText training corpus \citep{Gokaslan2019OpenWeb}\footnote{https://github.com/yet-another-account/openwebtext}. Our implementation details follow those of past work retraining GPT2 \citep{zellers2019defending}.




\subsection{Application: Paraphrasing}
\label{subsec:app_paraphrase}

%Paraphrasing is the most straightforward application for \method. \ari{The previous sentence gives you nothing.} 
Following \S\ref{subsec:reflective_decoder} the \decoder is learned in each direction (\lrRD, \rlRD) using the input sentence $s_{src}$. Then, $n_{\hat{s}}$ generations are sampled from both \lrRD and \rlRD: \
$$\hat{s}_1, ..., \hat{s}_{n_{\hat{s}}} \sim \text{\lrRD}, \hat{s}_{n_{\hat{s}} + 1}, ..., \hat{s}_{2*n_{\hat{s}} } \sim \text{\rlRD}$$

\noindent
This gives a robust set of candidates that could appear in the same left and right contexts as $s_{src}$. They are likely to be semantically related to $s_{src}$ but must be ranked to pick true paraphrases.
% We prioritize sentences with high semantic similarity to the input. 
\method is based on a notion of similarity centered on contextual distance (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). Thus we use the sum of expectations over forward and backward context ensembles as a final scoring function, leveraging the generated contexts of \lrRD and \rlRD:
%closely related to the \method sampling function (equation \ref{eqn:rd}), which aims to give high probability to contextually similar outputs, based on contextual distance posed as cross-entropy (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). While the sampling function attempts to estimate this with a reverse-direction LM, for final scoring we use a more robust estimate with the original context-generating LMs:
\begin{equation}
    score(\hat{s}) = \frac{1}{n_c}\sum_{c_{rh}} \text{\lrLM}(c_{rh}|\hat{s}) + \frac{1}{n_c}\sum_{c_{lh}} \text{\rlLM}(c_{lh}|\hat{s})
    \label{eqn:paraphrasing_full_score}
\end{equation}
\\
\noindent
where $c_{rh}$ are the generated contexts used in \rlRD, and $c_{lh}$ for \lrRD. This explicitly measures how well $\hat{s}$ fits into the potential contexts of $s_{src}$ because it is proportional to the expectation of a given paraphrase being generated by an ensemble of those forward and backward contexts. %\peter{will expand this a little}


%\ximing{if we want to save space, can we combine equation (2) and (3)? equation (3) seems to be a pretty straightforward step}
%\noindent
%taking the highest ranked one that differs sufficiently from $s_{src}$

\subsection{Application: Abductive Reasoning}
\label{subsec:app_anlg}

Abductive natural language generation ($\alpha$NLG from \citet{Bhagavatula2019AbductiveCR}) is the task of filling in the blank between 2 observations $o1$ and $o2$, with a hypothesis $h$ that abductively explains them. Approaching this problem unsupervised is challenging, particularly with unidirectional language models which cannot naturally condition on both sides when generating $h$. 

\method simplifies this problem. Using concatenated $o_1 + o_2$ as $s_{src}$ in Algorithm~\ref{alg}, we construct sampling functions \lrRD, \rlRD that capture the content of both observations. We are interested in sampling in between $o1$ and $o2$, so when sampling hypotheses $h$ from \rlRD we condition on the right-side observation $o_2$ (and vice-versa for \lrRD and $o_1$). This is equivalent to appending the given observation to sampled contexts: 
\begin{equation}
\begin{split}
    h_1, ..., h_{n_{\hat{s}}} &\sim \text{\rlRD}(h|o_2) \\ \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} &\sim \text{\lrRD}(h|o_1)
\end{split}
\end{equation}
%$$h_1, ..., h_{n_{\hat{s}}} \sim \text{\rlRD}(h|o_2) \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} \sim \text{\lrRD}(h|o_1)$$

Note that both \lrRD and \rlRD contain information about \textbf{both} $o_1$ and $o_2$, effectively turning a 2-sided contextual constraint into a 1-sided one. 

We also use a task-specific scoring function to rank sampled hypotheses. We would like a hypothesis $h$ that best explains both observations, and so use language models to measure this:
\begin{equation}
    score(h) = \text{\rlLM}(o1| h 
+ o2) + \text{\lrLM}(o2| o1 + h )
\label{eqn:anlg_score}
\end{equation}

Adding $h$ requires the LMs to ``explain'' each observation given the other, i.e. that $o2$ follows from $o1 + h$ and $o1$ from $h + o2$. To filter hypotheses that only explain one of the two observations, we remove any that make either observation less probable than the empty hypothesis, imposing:
\noindent
\begin{align*}
    \text{\rlLM}(o_1|h + o_2)>\text{\rlLM}(o_1|o_2) \\
    \text{\lrLM}(o_2|o_1 + h)>\text{\lrLM}(o_2|o_1)
\end{align*}
\subsection{Intuitions and Theory}
\label{subseq_intuitions_and_theory}
We motivate and derive \method as a way to sample generations that share contextual ``fit'' with a source text, deriving the sampling function of equation \ref{eqn:rd}. We start by considering how to compare a generation $\hat{s}$ with an input $s_{src}$. %We focus on unsupervised paraphrasing, \peter{Should qualify this a bit more "explain in terms of", not just generally "focus on"} which requires a notion of similarity to judge whether generation $\hat{s}$ is a paraphrase of source $s_{src}$. 

For the task of paraphrasing, we follow a distributional intuition \citep{firth1957synopsis}, that textual meaning can be understood by the contexts in which text appears. Many distributional approaches learn contentful neural representations by predicting context given input text \citep{word2vec,kiros2015skip}, then compare these representations to establish semantic similarity. We can, instead, compare contexts directly—judging the difference in meaning between texts $s_{src}$ and $\hat{s}$ by their divergence:
\begin{equation}
    D_{KL}(\text{\lrLM}(c|s_{src}), \text{\lrLM}(c|\hat{s}))
    \label{eqn:context_divergence}
\end{equation}
For simplicity, we use \lrLM to denote both the theoretical left-to-right distribution of text, and the model distribution estimating it. $\text{\lrLM}(c|s)$ is the distribution over right contexts $c$ given sentence s, so equation \ref{eqn:context_divergence} can be understood as how different the right-contexts we expect $s_{src}$ and $\hat{s}$ to appear in are. Note, while we use right-hand context here, this explanation symmetrically applies to left-hand. 

Measuring $D_{KL}$ exactly is infeasible, but for generation we are mainly interested in ranking or optimizing for this score (e.g. picking the best paraphrase $\hat{s}$). We take inspiration from language model training, using a finite sample estimate of cross-entropy as an effective proxy for $D_{KL}$:
\begin{equation}
\begin{split}
 \hat{H}(\text{\lrLM}(c|s_{src}), & \text{\lrLM}(c|\hat{s})) = \\ &\frac{1}{N}\sum_{c_i \sim \text{\lrLM}(c|s_{src})} -\text{log}\text{\lrLM}(c_i|\hat{s}) 
 \end{split}
 \label{eqn:reflective_scoring}
 \end{equation}
Where $c_i \sim \text{\lrLM}(c|s_{src})$ indicates contexts sampled from the LM conditioned on the input $s_{src}$.
%This allows us to leverage high-quality generations of our pretrained LMs. 
This objective makes intuitive sense: we want similar sentence $\hat{s}$ to rank highly, so we ``imagine'' likely contexts for $s_{src}$ and choose $\hat{s}$ that most generates these contexts. Optimal $\hat{s}$ fills approximately the same contextual hole as $s_{src}$, minimizing this ``contextual distance''. We explicitly test this notion for semantic equivalence in \S\ref{subsec_wmt18}.

In this form, $\hat{H}$ requires a fully generated $\hat{s}$ to compare to $s_{src}$, but we are trying to \textbf{generate} $\hat{s}$ for which the divergence from $s_{src}$ is low. We flip the role of ``text'' and ``context'' to define a function from which we can sample $\hat{s}$: 
\begin{equation}
    \begin{split}
    &\text{\rlRD}(\hat{s}_j|, \hat{s}_{j+1:n}) = \frac{ \prod_i  \text{\rlLM}(\hat{s}_j|\hat{s}_{j+1:n} + c_i)^{w_i}}{ \sum_{t \in V}  \prod_i  \text{\rlLM}(t|\hat{s}_{j+1:n} + c_i)^{w_i} }
    \end{split}
    \label{eqn:rd_theory}
\end{equation}
%\ximing{can we replace $t \in V$ with maybe $v \in V$ in equation (7) and (1)? $t$ denote timestep in many cases, we probably want to avoid it\\}
(equivalent to equation \ref{eqn:rd}, derived in \S\ref{app:derivation}) $\hat{s}_j$ is the $j^{th}$ token in $\hat{s}$ (sampled right-to-left from n to 0), and $V$ is the vocabulary. Weights $w_i$ are learned
%, aligning probability with contextual similarity to $s_{src}$ 
by maximizing the probability of $s_{src}$. 

Equation~\ref{eqn:rd_theory}, estimates the probability of \textit{predicting} $s_{src}$ and $\hat{s}$ from a finite set of contexts $c_i$ generated from $s_{src}$. This approximately minimizes~\ref{eqn:context_divergence} because, due to the sparsity of linguistic sequences, being generated by the same weighted ensemble of contexts strongly correlates with generating the same contexts in the same proportions, i.e. low divergence.
% Thus, we induce a sequential, token-wise probability distribution that approximately minimizes . 
We can sample $\hat{s}$ with low contextual distance from $s_{src}$ using \rlRD. Further, we can use left context to construct \lrRD by simply reversing the directions of the LMs used.


%\ari{We need to add more description of why the approximations (nucleus sampling forward, weight pruning backward) make sense.}

==> sections/backups/methods_1.tex <==
\section{Method}
\label{sec_method}

\subsection{Notation}
\label{subsec_notation}

Arrows indicate the order in which sampling functions condition on and generate tokens: $\xrightarrow{}$ indicates generating from the left-most token to the right (left-to-right), while $\xleftarrow{}$ indicates going right-to-left. For language models (LMs), this means \lrLM is what is often called a ``forward LM'', while \rlLM is a ``backward LM''. For the sampling function (RD), % \lrRD generates tokens left-to-right and \rlRD right-to-left. 
this also indicates which context is being conditioned on, e.g. \lrRD conditions on left context, and extends it to the right to generate output.
% \rlRD conditions on the right context, and generates backward (right-to-left). \lrLM and \rlLM are used together to score candidates, capturing bidirectional context.


\subsection{Overview} 
\label{subseq_overview}

Currently, LM-decoding is limited to a text \textit{continuation} paradigm. Given an input text $s_{input}$, $LM(c|s_{input})$ generates contexts $c$ that might come after (forward, i.e. \lrLM) or before (backward, i.e. \rlLM) the input. LM-decoding generates \textit{outside} of the input by continuing it, but many tasks require us to generate \textit{over} or \textit{within} the input: paraphrasing requires reformulating the input, while infilling requires inserting text in the middle of it. 

Reflective Decoding approaches this shortcoming by turning conventional LM-decoding around: $LM(c|s_{input})$ generates the kinds of contexts the input might appear in, while $RD(s)$ conditions on these generated contexts to model texts in the semantic neighborhood of $s_{input}$. Intuitively, this works because the input ($s_{input}$) is likely to appear in its own contexts by definition, but so should texts that might replace $s_{input}$ in-context. The distributional hypothesis \citep{firth1957synopsis} suggests semantically similar texts appear in similar contexts, making paraphrasing an exciting application. 

Concretely, 
%\method breaks out of text-continuation by applying it twice: first in one direction (e.g. forward with \lrLM in Figure \ref{fig_1}) 
\method first samples many possible contexts $c_i$ that could neighbor the input, e.g. using \lrLM in Figure \ref{fig_1}. This is the \textbf{\stepone}. Second, in the \textbf{\steptwo}, we apply a reverse-direction LM (\rlLM in Figure \ref{fig_1}) to extend the contexts back, generating text which fits in these contexts as well as $s_{input}$. To capture the collective meaning of all the $c_i$'s we  ensemble the different distributions imposed by conditioning on them:

\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{Z(s,c,w) }
    \label{eq:RD_simple}
\end{equation}
\noindent
where the $Z$ function simply normalizes for token-by-token generation (see equation \ref{eqn:rd} ). \lrRD is exactly the same, except it uses \lrLM with $c_i$'s generated by \rlLM. 


By taking an ensemble (Product of Experts \citep{hinton2002training}) between the contexts, we can generate $s$ that fits the full set of them. Importantly, weights $w_i$ are learned to prioritize the most informative contexts $c_i$. \peter{we can consider adding the ``weights learned to maximize $s_{input}$ because we \textit{know} it appears here'' intuition with pointers to 2.7, A.1, but maybe we want this somewhere else or nowhere? We should discuss}

The applicability of \method relies on contexts containing expressive information about the input to inform output $s$. To justify how generated contexts might do this, consider the paraphrasing example from Figure~\ref{fig_1} with input $s_{input}:$ \textit{How are circulatory system tissues formed?} Generated contexts reflect different aspects of $s_{input}$: $c_1$ situates $s_{input}$ as a question (\textit{This is a medical question...}), while $c_2$ and $c_3$ explore central concepts  (\textit{as with all tissue...}; \textit{about the circulatory system}). While each context could follow many sentences, together they form a fingerprint for $s_{input}$. A sentence that could be followed by all of $c_1,c_2,c_3$ will likely be a question ($c_1$) about tissue formation ($c_2$) and the circulatory system ($c_3$), and generally occupy the same semantic neighborhood as $s_{input}$: \textit{How do circulatory systems form?}

\peter{Then, last section connecting to infilling and other possible applications. I'm picturing this beginning something like "in paraphrasing, we are replacing all of $s_{input}$ with something that might appear in the same contexts. This is not necessary however, we might replace only part of a sentence (e.g. in context paraphrasing) or even insert text in a gap (text infilling) simply by holding part of $s_{input}$ static when we generate". Not sure if this is the best tactic though, I'm open to anything. }



\peter{JUST doing some brainstorming above, don't mind me
\peter{=============}}


Some contexts are more informative than others (i.e. probable but generic contexts like ``See the appendix for details.'' is not very informative), so we weight contexts based on informativeness to $s_{input}$. Weights $w_i$ are learned at inference-time to maximally produce the input $s_{input}$ under equation \ref{eq:RD_simple}. This can be seen as autoencoding, using weighted ensembles of contexts as a meaning representation.
These weights allow us to capture the semantics of $s_{input}$ by capturing how each context \textit{implies} $s_{input}$ as part of the ensemble (see \S\ref{subseq_intuitions_and_theory}, \S\ref{app:derivation}).

In the case of paraphrasing, we would like to replace the entire input. Thus, we simply sample from \rlRD (or the symmetric version, \lrRD from \S\ref{app:lr}), choosing the best output with bidirectional scoring (\S\ref{subsec:app_paraphrase}). 
In $\alpha$NLG the input is sentences $o_1,o_2$ and the task is to generate a third sentence that \textit{bridges} the narrative gap between them. Here, the challenge for LM-decoding is making use of context from both sides ($o_1$ on the left and $o_2$ on the right). \method allows us to generate 1-sided contexts that capture information about both $o_1$ and $o_2$, then replace the 0-length gap between them by appending $o_1$ and $o_2$ to the forward and backward context ensembles, respectively (\S\ref{subsec:app_anlg}). 

\subsection{\method}
\label{subsec:reflective_decoder}

\input{figs/algorithm_simple}


% We proceed to explicitly describe the steps to generate with \method, which requires an input text $s_{input}$, as well as forward and backward language models (\lrLM and \rlLM). From \S\ref{subseq_overview}, 
\method generates outputs that fit the same contexts as the input $s_{input}$, with the option to only overwrite a sub-span of $s_{input}$. By first generating representative contexts, then conditioning a language model in the reverse direction under a weighted ensemble of those contexts (equation \ref{eq:RD_simple}) we define the sampling function (RD), e.g \rlRD in Algorithm~\ref{alg}. For example, consider the right-hand context ensemble, keeping in mind that the process is repeated on the left-hand as well.

First, in the \textbf{\stepone} (line 1), we sample many right-hand contexts $c_i$ for $s_{input}$, using \lrLM. These will be used as a representative sample of the kind of contexts $s_{input}$ appears in.

Second, in the \textbf{\steptwo} (lines 2 - 3) our goal is to sample texts that appear in these same contexts. We construct the sampling function:
\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{ \prod_{j=0}^{|s|} \sum_{t \in V}  \prod_{i}  \text{\rlLM}(t|s_{j+1:|s|} + c_i)^{w_i} }
    \label{eqn:rd}
\end{equation}

\noindent
This is equivalent to equation \ref{eq:RD_simple}, substituting the exact normalization factor for $Z$. Equation~\ref{eqn:rd} is a token-wise Product of Experts model, that captures the semantic neighborhood of $s_{input}$ via the combination of contexts $c_i$ and their weights $w_i$ (\S\ref{subseq_intuitions_and_theory}). 
Our goal is to learn $w_i$ that maximize \rlRD$(s_{input})$, i.e. the probability of generating $s_{input}$. We initialize these weights (line 2),  then train them (line 3) using the Adam optimizer \citep{kingma2014adam}. We normalize weights to be a proper distribution at every step (see \S\ref{app:derivation}). Note, \lrRD is symmetrically learned in the reverse direction, flipping the roles of \lrLM and \rlLM and sampling left-hand context instead (see \S\ref{app:lr} for details).

Finally, we sample from \rlRD (and \lrRD), generating outputs that would appear in the same contexts as $s_{input}$. Depending on the application, we rank and select a final output in different ways. 


\input{figs/fig_examples}



\subsection{Implementation}
\label{subsec:implementation}

% Here, we cover implementation details for \S\ref{subsec:reflective_decoder}.

\paragraph{Weight Learning and Pruning} Weights $w_i$ are learned using the Adam optimizer \citep{kingma2014adam}. In practice this takes under 100 steps (negligible time compared to LM decoding). While we sample tens of contexts (line 1 of Algorithm~\ref{alg}), many end up with negligible weight under the learned distribution (equation \ref{eqn:rd}). To efficiently sample from this function, we drop all but the top $k_c$ contexts and renormalize weights: $k_c < n_c$ contexts are used during the \steptwo.
% described in \S\ref{subsec:reflective_decoder}. 


\paragraph{Parameters} We sample $n_c$ contexts to describe the source $s_{input}$. We use nucleus sampling \citep{Holtzman2019TheCC} with parameter $p_c$, and a maximum length of $len_c$. 
% As stated in \textbf{Weight Pruning}, we drop all but the top $k_c$ contexts by weight.
Once \lrRD and \rlRD are learned, we sample $n_{\hat{s}}$ generations from each, of length $len_{\hat{s}}$. We choose sampling  $p_{\hat{s}}$ per-example to account for vastly different entropy in RD (\S\ref{app:entropy_calibtration}). Values for all hyperparameters are available in \S\ref{app:model_params}.

\paragraph{Language Models} We train large forward (\lrLM) and backward (\rlLM) language models based on GPT2 \citep{radford2019gpt2}  using the OpenWebText training corpus \citep{Gokaslan2019OpenWeb}\footnote{https://github.com/yet-another-account/openwebtext}. Our implementation details follow those of past work retraining GPT2 \citep{zellers2019defending}.




\subsection{Application: Paraphrasing}
\label{subsec:app_paraphrase}

%Paraphrasing is the most straightforward application for \method. \ari{The previous sentence gives you nothing.} 
Following \S\ref{subsec:reflective_decoder} the \decoder is learned in each direction (\lrRD, \rlRD) using the input sentence $s_{input}$. Then, $n_{\hat{s}}$ generations are sampled from both \lrRD and \rlRD: \
$$\hat{s}_1, ..., \hat{s}_{n_{\hat{s}}} \sim \text{\lrRD}, \hat{s}_{n_{\hat{s}} + 1}, ..., \hat{s}_{2*n_{\hat{s}} } \sim \text{\rlRD}$$

\noindent
This gives a robust set of candidates that could appear in the same left and right contexts as $s_{input}$. They are likely to be semantically related to $s_{input}$ but must be ranked to pick true paraphrases.
% We prioritize sentences with high semantic similarity to the input. 
\method is based on a notion of similarity centered on contextual distance (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). Thus we use the sum of expectations over forward and backward context ensembles as a final scoring function, leveraging the generated contexts of \lrRD and \rlRD:
%closely related to the \method sampling function (equation \ref{eqn:rd}), which aims to give high probability to contextually similar outputs, based on contextual distance posed as cross-entropy (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). While the sampling function attempts to estimate this with a reverse-direction LM, for final scoring we use a more robust estimate with the original context-generating LMs:
\begin{equation}
    score(\hat{s}) = \frac{1}{n_c}\sum_{c_{rh}} \text{\lrLM}(c_{rh}|\hat{s}) + \frac{1}{n_c}\sum_{c_{lh}} \text{\rlLM}(c_{lh}|\hat{s})
    \label{eqn:paraphrasing_full_score}
\end{equation}
\\
\noindent
where $c_{rh}$ are the generated contexts used in \rlRD, and $c_{lh}$ for \lrRD. This explicitly measures how well $\hat{s}$ fits into the potential contexts of $s_{input}$ because it is proportional to the expectation of a given paraphrase being generated by an ensemble of those forward and backward contexts. %\peter{will expand this a little}


%\ximing{if we want to save space, can we combine equation (2) and (3)? equation (3) seems to be a pretty straightforward step}
%\noindent
%taking the highest ranked one that differs sufficiently from $s_{input}$

\subsection{Application: Abductive Reasoning}
\label{subsec:app_anlg}

Abductive natural language generation ($\alpha$NLG from \citet{Bhagavatula2019AbductiveCR}) is the task of filling in the blank between 2 observations $o1$ and $o2$, with a hypothesis $h$ that abductively explains them. Approaching this problem unsupervised is challenging, particularly with unidirectional language models which cannot naturally condition on both sides when generating $h$. 

\method simplifies this problem. Using concatenated $o_1 + o_2$ as $s_{input}$ in Algorithm~\ref{alg}, we construct sampling functions \lrRD, \rlRD that capture the content of both observations. We are interested in sampling in between $o1$ and $o2$, so when sampling hypotheses $h$ from \rlRD we condition on the right-side observation $o_2$ (and vice-versa for \lrRD and $o_1$). This is equivalent to appending the given observation to sampled contexts: 
\begin{equation}
\begin{split}
    h_1, ..., h_{n_{\hat{s}}} &\sim \text{\rlRD}(h|o_2) \\ \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} &\sim \text{\lrRD}(h|o_1)
\end{split}
\end{equation}
%$$h_1, ..., h_{n_{\hat{s}}} \sim \text{\rlRD}(h|o_2) \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} \sim \text{\lrRD}(h|o_1)$$

Note that both \lrRD and \rlRD contain information about \textbf{both} $o_1$ and $o_2$, effectively turning a 2-sided contextual constraint into a 1-sided one. 

We also use a task-specific scoring function to rank sampled hypotheses. We would like a hypothesis $h$ that best explains both observations, and so use language models to measure this:
\begin{equation}
    score(h) = \text{\rlLM}(o1| h 
+ o2) + \text{\lrLM}(o2| o1 + h )
\label{eqn:anlg_score}
\end{equation}

Adding $h$ requires the LMs to ``explain'' each observation given the other, i.e. that $o2$ follows from $o1 + h$ and $o1$ from $h + o2$. To filter hypotheses that only explain one of the two observations, we remove any that make either observation less probable than the empty hypothesis, imposing:
\noindent
\begin{align*}
    \text{\rlLM}(o_1|h + o_2)>\text{\rlLM}(o_1|o_2) \\
    \text{\lrLM}(o_2|o_1 + h)>\text{\lrLM}(o_2|o_1)
\end{align*}
\subsection{Intuitions and Theory}
\label{subseq_intuitions_and_theory}
We motivate and derive \method as a way to sample generations that share contextual ``fit'' with a source text, deriving the sampling function of equation \ref{eqn:rd}. We start by considering how to compare a generation $\hat{s}$ with an input $s_{input}$. %We focus on unsupervised paraphrasing, \peter{Should qualify this a bit more "explain in terms of", not just generally "focus on"} which requires a notion of similarity to judge whether generation $\hat{s}$ is a paraphrase of source $s_{input}$. 

For the task of paraphrasing, we follow a distributional intuition \citep{firth1957synopsis}, that textual meaning can be understood by the contexts in which text appears. Many distributional approaches learn contentful neural representations by predicting context given input text \citep{word2vec,kiros2015skip}, then compare these representations to establish semantic similarity. We can, instead, compare contexts directly—judging the difference in meaning between texts $s_{input}$ and $\hat{s}$ by their divergence:
\begin{equation}
    D_{KL}(\text{\lrLM}(c|s_{input}), \text{\lrLM}(c|\hat{s}))
    \label{eqn:context_divergence}
\end{equation}
For simplicity, we use \lrLM to denote both the theoretical left-to-right distribution of text, and the model distribution estimating it. $\text{\lrLM}(c|s)$ is the distribution over right contexts $c$ given sentence s, so equation \ref{eqn:context_divergence} can be understood as how different the right-contexts we expect $s_{input}$ and $\hat{s}$ to appear in are. Note, while we use right-hand context here, this explanation symmetrically applies to left-hand. 

Measuring $D_{KL}$ exactly is infeasible, but for generation we are mainly interested in ranking or optimizing for this score (e.g. picking the best paraphrase $\hat{s}$). We take inspiration from language model training, using a finite sample estimate of cross-entropy as an effective proxy for $D_{KL}$:
\begin{equation}
\begin{split}
 \hat{H}(\text{\lrLM}(c|s_{input}), & \text{\lrLM}(c|\hat{s})) = \\ &\frac{1}{N}\sum_{c_i \sim \text{\lrLM}(c|s_{input})} -\text{log}\text{\lrLM}(c_i|\hat{s}) 
 \end{split}
 \label{eqn:reflective_scoring}
 \end{equation}
Where $c_i \sim \text{\lrLM}(c|s_{input})$ indicates contexts sampled from the LM conditioned on the input $s_{input}$.
%This allows us to leverage high-quality generations of our pretrained LMs. 
This objective makes intuitive sense: we want similar sentence $\hat{s}$ to rank highly, so we ``imagine'' likely contexts for $s_{input}$ and choose $\hat{s}$ that most generates these contexts. Optimal $\hat{s}$ fills approximately the same contextual hole as $s_{input}$, minimizing this ``contextual distance''. We explicitly test this notion for semantic equivalence in \S\ref{subsec_wmt18}.

In this form, $\hat{H}$ requires a fully generated $\hat{s}$ to compare to $s_{input}$, but we are trying to \textbf{generate} $\hat{s}$ for which the divergence from $s_{input}$ is low. We flip the role of ``text'' and ``context'' to define a function from which we can sample $\hat{s}$: 
\begin{equation}
    \begin{split}
    &\text{\rlRD}(\hat{s}_j|, \hat{s}_{j+1:n}) = \frac{ \prod_i  \text{\rlLM}(\hat{s}_j|\hat{s}_{j+1:n} + c_i)^{w_i}}{ \sum_{t \in V}  \prod_i  \text{\rlLM}(t|\hat{s}_{j+1:n} + c_i)^{w_i} }
    \end{split}
    \label{eqn:rd_theory}
\end{equation}
%\ximing{can we replace $t \in V$ with maybe $v \in V$ in equation (7) and (1)? $t$ denote timestep in many cases, we probably want to avoid it\\}
(equivalent to equation \ref{eqn:rd}, derived in \S\ref{app:derivation}) $\hat{s}_j$ is the $j^{th}$ token in $\hat{s}$ (sampled right-to-left from n to 0), and $V$ is the vocabulary. Weights $w_i$ are learned
%, aligning probability with contextual similarity to $s_{input}$ 
by maximizing the probability of $s_{input}$. 

Equation~\ref{eqn:rd_theory}, estimates the probability of \textit{predicting} $s_{input}$ and $\hat{s}$ from a finite set of contexts $c_i$ generated from $s_{input}$. This approximately minimizes~\ref{eqn:context_divergence} because, due to the sparsity of linguistic sequences, being generated by the same weighted ensemble of contexts strongly correlates with generating the same contexts in the same proportions, i.e. low divergence.
% Thus, we induce a sequential, token-wise probability distribution that approximately minimizes . 
We can sample $\hat{s}$ with low contextual distance from $s_{input}$ using \rlRD. Further, we can use left context to construct \lrRD by simply reversing the directions of the LMs used.


%\ari{We need to add more description of why the approximations (nucleus sampling forward, weight pruning backward) make sense.}

==> sections/backups/methods_3.tex <==
\section{Method}
\label{sec_method}

\subsection{Notation}
\label{subsec_notation}

Arrows indicate the order in which sampling functions condition on and generate tokens: $\xrightarrow{}$ indicates generating from the left-most token to the right (left-to-right), while $\xleftarrow{}$ indicates going right-to-left. For language models (LMs), this means \lrLM is what is often called a ``forward LM'', while \rlLM is a ``backward LM''. For our sampling function (RD), % \lrRD generates tokens left-to-right and \rlRD right-to-left. 
this also indicates which context is being conditioned on, e.g. \lrRD conditions on left context, and extends it to the right to generate output.
% \rlRD conditions on the right context, and generates backward (right-to-left). \lrLM and \rlLM are used together to score candidates, capturing bidirectional context.


\subsection{Overview} 
\label{subseq_overview}

Currently, LM-decoding is limited to a \textit{text continuation} paradigm. Given an input text $s_{input}$, $\text{LM}(c|s_{input})$ generates contexts $c$ that might come after (forward, i.e. \lrLM) or before (backward, i.e. \rlLM) the input. LM-decoding generates \textit{outside} of the input by continuing it, but many tasks require us to generate \textit{over} or \textit{within} the input: paraphrasing requires reformulating the input, while infilling requires inserting text in the middle of it. 

\peter{** trying something. Previous version is commented out.}

Reflective Decoding approaches this shortcoming by turning conventional LM-decoding around: while $\text{LM}(c|s_{input})$ generates the kinds of contexts the input might appear in, $RD(s)$ instead conditions on these generated contexts to model texts $s$ in the semantic neighborhood of $s_{input}$. Intuitively, this works because $s_{input}$ is likely to appear in its own contexts by definition, but so should texts that might replace $s_{input}$ in-context. The distributional hypothesis \citep{firth1957synopsis} suggests semantically similar texts appear in similar contexts, making paraphrasing an exciting application. 

Concretely, 
%\method breaks out of text-continuation by applying it twice: first in one direction (e.g. forward with \lrLM in Figure \ref{fig_1}) 
\method first samples many possible contexts $c_i$ that could neighbor the input, e.g. using \lrLM in Figure \ref{fig_1}. This is the \textbf{\stepone}. Second, in the \textbf{\steptwo}, we apply a reverse-direction LM (\rlLM in Figure \ref{fig_1}) to extend the contexts back, generating text which fits in these contexts as well as $s_{input}$ fits them. To consider all $c_i$'s while decoding, we ensemble the different distributions imposed by conditioning on each $c_i$:%capture the collective meaning of all the $c_i$'s we ensemble the different distributions imposed by conditioning on each $c_i$:

\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{Z(s,c,w) }
    \label{eq:RD_simple}
\end{equation}
\noindent
where $Z$ normalizes to a proper probability distribution (see equation \ref{eqn:rd} ). Reversed \lrRD is the same, except it uses \lrLM with $c_i$'s generated by \rlLM. 


By ensembling the contexts in a Product of Experts \citep{hinton2002training} framework, we can generate a hypothesis $s$ that fits the full contextual fingerprint. Yet, some contexts are more informative than others:  probable but generic contexts like ``See the appendix for details.'' are not very informative. We learn weights $w_i$ to prioritize the most informative contexts $c_i$, by maximizing the probability of $s_{input}$ under equation \ref{eq:RD_simple}, as described in Algorithm~\ref{alg}. In essence, we learn an on-the-fly autoencoder at inference time, using weighted ensembles of contexts as a meaning representation (see \S\ref{subseq_intuitions_and_theory}, \S\ref{app:derivation}).
% These weights allow us to capture the semantics of $s_{input}$ by capturing how each context \textit{implies} $s_{input}$ as part of the ensemble (see \S\ref{subseq_intuitions_and_theory}, \S\ref{app:derivation}).

% The applicability of \method relies on contexts containing expressive information about the input to inform output $s$. 
To motivate how this method functions, consider the paraphrasing example from Figure~\ref{fig_1} with input $s_{input}:$ \textit{How are circulatory system tissues formed?} Generated contexts reflect different aspects of $s_{input}$: $c_1$ situates $s_{input}$ as a question (\textit{This is a medical question...}), while $c_2$ and $c_3$ explore central concepts  (\textit{as with all tissue...}; \textit{about the circulatory system}). Even though each context could follow many sentences, together they form a fingerprint for $s_{input}$. A sentence that could be followed by all of $c_1,c_2,c_3$ will likely be a question ($c_1$) about tissue formation ($c_2$) and the circulatory system ($c_3$), and generally occupy the same semantic neighborhood as $s_{input}$: e.g. \textit{How do circulatory systems form?}

%\peter{Then, last section connecting to infilling and other possible applications. I'm picturing this beginning something like "in paraphrasing, we are replacing all of $s_{input}$ with something that might appear in the same contexts. This is not necessary however, we might replace only part of a sentence (e.g. in context paraphrasing) or even insert text in a gap (text infilling) simply by holding part of $s_{input}$ static when we generate". Not sure if this is the best tactic though, I'm open to anything. }

In the case of paraphrasing, our task is to replace all of $s_{input}$ with something that might appear in the same contexts. Other tasks, however, might require us to replace only part of a sentence (e.g. in-context paraphrasing) or even insert text at a given position (e.g. infilling). \method makes this easy: simply hold part of $s_{input}$ static when we generate from RD.

% In the case of paraphrasing, we would like to replace the entire input. Thus, we simply sample from \rlRD (or the symmetric version, \lrRD from \S\ref{app:lr}), choosing the best output with bidirectional scoring (\S\ref{subsec:app_paraphrase}). 
% In $\alpha$NLG the input is sentences $o_1,o_2$ and the task is to generate a third sentence that \textit{bridges} the narrative gap between them. Here, the challenge for LM-decoding is making use of context from both sides ($o_1$ on the left and $o_2$ on the right). \method allows us to generate 1-sided contexts that capture information about both $o_1$ and $o_2$, then replace the 0-length gap between them by appending $o_1$ and $o_2$ to the forward and backward context ensembles, respectively (\S\ref{subsec:app_anlg}). 

\subsection{\method}
\label{subsec:reflective_decoder}

\input{figs/algorithm_simple}


% We proceed to explicitly describe the steps to generate with \method, which requires an input text $s_{input}$, as well as forward and backward language models (\lrLM and \rlLM). From \S\ref{subseq_overview}, 
% \method generates outputs that fit the same contexts as the input $s_{input}$, with the option to only overwrite a sub-span of $s_{input}$. % By first generating representative contexts, then conditioning a language model in the reverse direction under a weighted ensemble of those contexts (equation \ref{eq:RD_simple}) we define the sampling function (RD), e.g \rlRD in Algorithm~\ref{alg}.
Let's dive into the details of \method, by considering the right-hand context ensemble (\rlRD), keeping in mind that the process is repeated on the left-hand as well (\lrRD). 


First, in the \textbf{\stepone} (line 1 of Algorithm~\ref{alg}), we sample many right-hand contexts $c_i$ for $s_{input}$, using \lrLM. These will be used as a representative sample of the contexts $s_{input}$ appears in.
Second, in the \textbf{\steptwo} (lines 2 \& 3) our goal is to construct a sampling function \rlRD that will yield texts similar to $s_{input}$. We define \lrRD as:
\begin{equation}
    \text{\rlRD}(s) = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{ \prod_{j=0}^{|s|} \sum_{t \in V}  \prod_{i}  \text{\rlLM}(t|s_{j+1:|s|} + c_i)^{w_i} }
    \label{eqn:rd}
\end{equation}

\noindent
This is equivalent to equation \ref{eq:RD_simple}, but giving the exact normalization factor $Z$. 

Equation~\ref{eqn:rd} is a token-wise Product of Experts model, that captures the semantic neighborhood of $s_{input}$ via the combination of contexts $c_i$ and their weights $w_i$ (\S\ref{subseq_intuitions_and_theory}). 
We learn $w_i$ that maximize $\text{\rlRD}(s_{input})$, i.e. the probability of generating $s_{input}$. We initialize these weights (line 2),  then train them (line 3) using the Adam optimizer \citep{kingma2014adam}. We normalize weights into a proper distribution at every step (see \S\ref{app:derivation}). 

\lrRD is symmetrically learned in the reverse direction, flipping the roles of \lrLM and \rlLM and sampling left-hand context instead (see \S\ref{app:lr} for details). Finally, we generate from \rlRD (and \lrRD), sampling outputs that would appear in the same contexts as $s_{input}$. Depending on the application, we rank and select a final output in different ways, always using \lrLM and \rlLM together to capture bidirectional fit.


\input{figs/fig_examples}



\subsection{Implementation}
\label{subsec:implementation}

% Here, we cover implementation details for \S\ref{subsec:reflective_decoder}.

\paragraph{Weight Learning and Pruning} Context weights $w_i$ are learned using the Adam optimizer \citep{kingma2014adam}. In practice this takes under 100 steps (negligible time compared to LM decoding). While we sample tens of contexts (line 1 of Algorithm~\ref{alg}), many end up with negligible weight under the learned distribution (equation \ref{eqn:rd}). To efficiently sample from this function, we drop all but the top $k_c$ contexts and renormalize weights: $k_c < n_c$ contexts are used during the \steptwo.
% described in \S\ref{subsec:reflective_decoder}. 


\paragraph{Parameters} We sample $n_c$ contexts to describe the source $s_{input}$. We use nucleus sampling \citep{Holtzman2019TheCC} with parameter $p_c$, and a maximum length of $len_c$. 
% As stated in \textbf{Weight Pruning}, we drop all but the top $k_c$ contexts by weight.
Once \lrRD and \rlRD are learned, we sample $n_{s}$ generations from each, of length $len_{s}$. We again use nucleus sampling, but choose $p_{s}$ per-example to account for vastly different entropy in RD (\S\ref{app:entropy_calibtration}). Values for all hyperparameters are available in \S\ref{app:model_params}.

\paragraph{Language Models} We train large forward (\lrLM) and backward (\rlLM) language models based on GPT-2 \citep{radford2019gpt2}  using the OpenWebText training corpus \citep{Gokaslan2019OpenWeb}\footnote{https://github.com/yet-another-account/openwebtext}. Our implementation details follow those of past work retraining GPT-2 \citep{zellers2019defending}.




\subsection{Application: Paraphrasing}
\label{subsec:app_paraphrase}

%Paraphrasing is the most straightforward application for \method. \ari{The previous sentence gives you nothing.} 
To paraphrase, we begin by generating candidate outputs. Following \S\ref{subsec:reflective_decoder} the \decoder is learned in each direction (\lrRD, \rlRD) using the input sentence $s_{input}$. Then, $n_{s}$ generations are sampled from both \lrRD and \rlRD: \
$$s_1, ..., s_{n_s} \sim \text{\lrRD}, s_{n_s + 1}, ..., s_{2*n_{s} } \sim \text{\rlRD}$$
%$$\hat{s}_1, ..., \hat{s}_{n_{\hat{s}}} \sim \text{\lrRD}, \hat{s}_{n_{\hat{s}} + 1}, ..., \hat{s}_{2*n_{\hat{s}} } \sim \text{\rlRD}$$

\noindent
This gives a robust set of candidates that are compatible with the same left and right contexts as $s_{input}$. Most of these are semantically related to $s_{input}$, but must be scored and ranked in order to select true paraphrases.
% We prioritize sentences with high semantic similarity to the input. 
\method is based on a notion of similarity centered on contextual distance (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). Thus we use the sum of expectations over forward and backward context ensembles as a final scoring function, leveraging the generated contexts of \lrRD and \rlRD:
%closely related to the \method sampling function (equation \ref{eqn:rd}), which aims to give high probability to contextually similar outputs, based on contextual distance posed as cross-entropy (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). While the sampling function attempts to estimate this with a reverse-direction LM, for final scoring we use a more robust estimate with the original context-generating LMs:
\begin{equation}
    score(s) = \frac{1}{n_c}\sum_{c_{rh}} \text{\lrLM}(c_{rh}|s) + \frac{1}{n_c}\sum_{c_{lh}} \text{\rlLM}(c_{lh}|s)
    \label{eqn:paraphrasing_full_score}
\end{equation}
%\begin{equation}
%    score(\hat{s}) = \frac{1}{n_c}\sum_{c_{rh}} \text{\lrLM}(c_{rh}|\hat{s}) + \frac{1}{n_c}\sum_{c_{lh}} \text{\rlLM}(c_{lh}|\hat{s})
%    \label{eqn:paraphrasing_full_score}
%\end{equation}
\\
\noindent
where $c_{rh}$ are the generated contexts used in \rlRD, and $c_{lh}$ for \lrRD. This explicitly measures how well a candidate $s$ fits into the potential contexts of $s_{input}$ because it is proportional to the expectation of a given paraphrase being generated by an ensemble of those forward and backward contexts. %\peter{will expand this a little}


%\ximing{if we want to save space, can we combine equation (2) and (3)? equation (3) seems to be a pretty straightforward step}
%\noindent
%taking the highest ranked one that differs sufficiently from $s_{input}$

\subsection{Application: Abductive Reasoning}
\label{subsec:app_anlg}



Abductive natural language generation ($\alpha$NLG from \citet{Bhagavatula2019AbductiveCR}) is the task of filling in the blank between 2 observations $o1$ and $o2$, with a hypothesis $h$ that abductively explains them. The challenge for LM-decoding is making use of context from both sides ($o_1$ on the left and $o_2$ on the right). This is particularly challenging for unsupervised methods because unidirectional language models cannot naturally condition on both sides when generating $h$. 

\method simplifies this problem by generating 1-sided contexts that capture information about both $o_1$ and $o_2$, then appending $o_1$ and $o_2$ to the forward and backward context ensembles, respectively. %(\S\ref{subsec:app_anlg}). 
Concretely, we use concatenated $o_1 + o_2$ as $s_{input}$ in Algorithm~\ref{alg}, and construct sampling functions \lrRD, \rlRD informed by both observations. 
We are interested in sampling in between $o1$ and $o2$, so when sampling hypotheses $h$ from \rlRD we condition on the right-side observation $o_2$ (and vice-versa for \lrRD and $o_1$). This is equivalent to appending the given observation to sampled contexts: 
\begin{equation}
\begin{split}
    h_1, ..., h_{n_{\hat{s}}} &\sim \text{\rlRD}(h|o_2) \\ \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} &\sim \text{\lrRD}(h|o_1)
\end{split}
\end{equation}
%$$h_1, ..., h_{n_{\hat{s}}} \sim \text{\rlRD}(h|o_2) \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} \sim \text{\lrRD}(h|o_1)$$

Note that both \lrRD and \rlRD contain information about \textbf{both} $o_1$ and $o_2$, effectively turning a 2-sided contextual constraint into a 1-sided one. 

We also use a task-specific scoring function to rank sampled hypotheses. We would like a hypothesis $h$ that best explains both observations, and so use language models to measure this:
\begin{equation}
    score(h) = \text{\rlLM}(o1| h 
+ o2) + \text{\lrLM}(o2| o1 + h )
\label{eqn:anlg_score}
\end{equation}

Adding $h$ should help to ``explain'' each observation given the other, i.e. that $o2$ follows from $o1 + h$ and $o1$ from $h + o2$. To filter hypotheses that only explain one of the two observations, we remove any that make either observation less probable than the empty hypothesis, imposing:
\noindent
\begin{align*}
    \text{\rlLM}(o_1|h + o_2)>\text{\rlLM}(o_1|o_2) \\
    \text{\lrLM}(o_2|o_1 + h)>\text{\lrLM}(o_2|o_1)
\end{align*}
\subsection{Intuitions and Theory}
\label{subseq_intuitions_and_theory}
Here, we discuss the theoretical intuition for \method, as a way to sample generations that share contextual ``fit'' with a source text, deriving the sampling function of equation \ref{eqn:rd}. We start by considering how to compare a generation $s$ with an input $s_{input}$. %We focus on unsupervised paraphrasing, \peter{Should qualify this a bit more "explain in terms of", not just generally "focus on"} which requires a notion of similarity to judge whether generation $\hat{s}$ is a paraphrase of source $s_{input}$. 

For the task of paraphrasing, we follow a distributional intuition \citep{firth1957synopsis}, that textual meaning can be understood by the contexts in which text appears. Many distributional approaches learn contentful neural representations by predicting context given input text \citep{word2vec,kiros2015skip}, then compare these representations to establish semantic similarity. We can, instead, compare contexts directly—judging the difference in meaning between texts $s_{input}$ and $s$ by their divergence:
\begin{equation}
    D_{KL}(\text{\lrLM}(c|s_{input}), \text{\lrLM}(c|\hat{s}))
    \label{eqn:context_divergence}
\end{equation}
We use \lrLM to interchangeably denote the theoretical left-to-right distribution of text, and the LM estimating it. Thus, $\text{\lrLM}(c|s)$ is the distribution over right contexts $c$ given sentence s, and equation \ref{eqn:context_divergence} can be understood as the ``information difference'' we expect $s$ to have from $s_{input}$. Note, we could similarly use left-hand context and \rlLM. 

Measuring $D_{KL}$ exactly is infeasible, but for generation we are mainly interested in ranking by this score (e.g. picking the best paraphrase $s$). Thus, as in language model training—we use a finite sample estimate of cross-entropy as an effective proxy for $D_{KL}$:
\begin{equation}
\begin{split}
 \hat{H}(\text{\lrLM}(c|s_{input}), & \text{\lrLM}(c|s)) = \\ &\frac{1}{N}\sum_{c_i \sim \text{\lrLM}(c|s_{input})} -\text{log}\text{\lrLM}(c_i|s) 
 \end{split}
 \label{eqn:reflective_scoring}
 \end{equation}
Where $c_i \sim \text{\lrLM}(c|s_{input})$ indicates contexts for $s_{input}$ generated by the LM.
%This allows us to leverage high-quality generations of our pretrained LMs. 
Intuitively, we want to minimize this score when generating $s$: optimal $s$ has a similar meaning to $s_{input}$ and so fills approximately the same contextual hole as, minimizing the value of this ``contextual distance''. We explicitly test this notion for semantic equivalence in \S\ref{subsec_wmt18}.

In this form, $\hat{H}$ requires a fully generated $s$ to compare to $s_{input}$, but we are trying to \textbf{generate} $s$ for which the divergence from $s_{input}$ is low. We flip the role of ``text'' and ``context'' to define a function from which we can sample $s$: 
\begin{equation}
    \begin{split}
    &\text{\rlRD}(s_j|, s_{j+1:n}) = \frac{ \prod_i  \text{\rlLM}(s_j|s_{j+1:n} + c_i)^{w_i}}{ \sum_{t \in V}  \prod_i  \text{\rlLM}(t|s_{j+1:n} + c_i)^{w_i} }
    \end{split}
    \label{eqn:rd_theory}
\end{equation}
%\ximing{can we replace $t \in V$ with maybe $v \in V$ in equation (7) and (1)? $t$ denote timestep in many cases, we probably want to avoid it\\}
(equivalent to equation \ref{eqn:rd}, derived in \S\ref{app:derivation}) $s_j$ is the $j^{th}$ token in $s$ (sampled right-to-left from n to 0), and $V$ is the vocabulary. Weights $w_i$ are learned
%, aligning probability with contextual similarity to $s_{input}$ 
by maximizing the probability of $s_{input}$. 

Equation~\ref{eqn:rd_theory}, estimates the probability of \textit{predicting} $s_{input}$ and $s$ from a finite set of contexts $c_i$ generated from $s_{input}$. This approximately minimizes~\ref{eqn:context_divergence} because, due to the sparsity of linguistic sequences, being generated by the same weighted ensemble of contexts strongly correlates with generating the same contexts in the same proportions, i.e. low divergence.
% Thus, we induce a sequential, token-wise probability distribution that approximately minimizes . 
We can sample $s$ with low contextual distance from $s_{input}$ using \rlRD. Further, we can use left context to construct \lrRD by simply reversing the directions of the LMs used.


%\ari{We need to add more description of why the approximations (nucleus sampling forward, weight pruning backward) make sense.}

==> sections/backups/methods_4.tex <==
\section{Method}
\label{sec_method}

\subsection{Notation}
\label{subsec_notation}

Arrows indicate the order in which sampling functions condition on and generate tokens: $\xrightarrow{}$ indicates generating from the left-most token to the right (left-to-right), while $\xleftarrow{}$ indicates going right-to-left. For language models (LMs), this means \lrLM is what is often called a ``forward LM'', while \rlLM is a ``backward LM''. For our sampling function (RD), % \lrRD generates tokens left-to-right and \rlRD right-to-left. 
this also indicates which context is being conditioned on, e.g. \lrRD conditions on left context, and extends it to the right to generate output.
% \rlRD conditions on the right context, and generates backward (right-to-left). \lrLM and \rlLM are used together to score candidates, capturing bidirectional context.


\subsection{Overview} 
\label{subseq_overview}

Currently, LM-decoding is limited to a \textit{text continuation} paradigm. Given an input text $s_{input}$, $\text{LM}(c|s_{input})$ generates contexts $c$ that might come after (forward, i.e. \lrLM) or before (backward, i.e. \rlLM) the input. LM-decoding generates \textit{outside} of the input by continuing it, but many tasks require us to generate \textit{over} or \textit{within} the input: paraphrasing requires reformulating the input, while infilling requires inserting text in the middle of it. 

\peter{**}
Reflective Decoding approaches this shortcoming by turning conventional LM-decoding around: while $\text{LM}(c|s_{input})$ generates the kinds of contexts the input might appear in, $\text{RD}(s)$ generates $s$ that might appear in those same contexts. $RD(s_{input})$ will be high for instance: $s_{input}$ is likely to appear in its own contexts by definition. Other text $s$ will be likely too; the distributional hypothesis \citep{firth1957synopsis} suggests semantically similar texts appear in similar contexts, meaning $\text{RD}(s)$ is also likely to sample in the semantic neighborhood of $s_{input}$. Paraphrasing is an exciting application. 

Concretely, \method samples $s$ that fits the same context as $s_{input}$ in 2 simple steps. First, LM-decoding is used to sample a set of \textit{representative} contexts $c_i$ (e.g. sampling rh contexts with \lrLM in Figure~\ref{fig_1}). This is the \textbf{\stepone}, which gives concrete examples of the kinds of contexts $s_{input}$ appears in. Next, we generate text that fits these contexts, simply using a reverse direction LM (\rlLM in Figure~\ref{fig_1}) to sample back in an ensemble:

\begin{equation}
    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{Z(s,c,w) }
    \label{eq:RD_simple}
\end{equation}
\noindent
In effect, text $s$ that is a good fit for all contexts $c_i$ will be likely. This is the \textbf{\steptwo}. $Z$ here normalizes to a proper probability distribution (see equation \ref{eqn:rd} ), and weights $w_i$ prioritize especially informative contexts. Note, reversed \lrRD is the same, but using \lrLM with $c_i$ generated by \rlLM. 

By ensembling the contexts in a Product of Experts \citep{hinton2002training}, we can generate a hypothesis $s$ that fits the full contextual fingerprint of $s_{input}$. Yet, some contexts are more informative than others:  probable but generic contexts like ``See the appendix for details.'' are not very informative. We learn weights $w_i$ to prioritize the most informative contexts $c_i$, by maximizing the probability of $s_{input}$ under equation \ref{eq:RD_simple} (Algorithm~\ref{alg}). Intuitively, $s_{input}$ should be likely as it fits in its own context. Technically, we learn an on-the-fly autoencoder at inference time, using weighted ensembles of contexts as a representation (see \S\ref{subseq_intuitions_and_theory}, \S\ref{app:derivation}).

%Reflective Decoding approaches this shortcoming by turning conventional LM-decoding around: while $\text{LM}(c|s_{input})$ generates the kinds of contexts the input might appear in, $RD(s)$ instead conditions on these generated contexts to model texts $s$ in the semantic neighborhood of $s_{input}$. Intuitively, this works because $s_{input}$ is likely to appear in its own contexts by definition, but so should texts that might replace $s_{input}$ in-context. The distributional hypothesis \citep{firth1957synopsis} suggests semantically similar texts appear in similar contexts, making paraphrasing an exciting application. 

%Concretely, 
%\method first samples many possible contexts $c_i$ that could neighbor the input, e.g. using \lrLM in Figure \ref{fig_1}. This is the \textbf{\stepone}. Second, in the \textbf{\steptwo}, we apply a reverse-direction LM (\rlLM in Figure \ref{fig_1}) to extend the contexts back, generating text which fits in these contexts as well as $s_{input}$ fits them. To consider all $c_i$'s while decoding, we ensemble the different distributions imposed by conditioning on each $c_i$:

%\begin{equation}
%    \text{\rlRD(s)} = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{Z(s,c,w) }
%    \label{eq:RD_simple}
%\end{equation}
%\noindent
%where $Z$ normalizes to a proper probability distribution (see equation \ref{eqn:rd} ). Reversed \lrRD is the same, except it uses \lrLM with $c_i$'s generated by \rlLM. 


%By ensembling the contexts in a Product of Experts \citep{hinton2002training} framework, we can generate a hypothesis $s$ that fits the full contextual fingerprint. Yet, some contexts are more informative than others:  probable but generic contexts like ``See the appendix for details.'' are not very informative. We learn weights $w_i$ to prioritize the most informative contexts $c_i$, by maximizing the probability of $s_{input}$ under equation \ref{eq:RD_simple}, as described in Algorithm~\ref{alg}. In essence, we learn an on-the-fly autoencoder at inference time, using weighted ensembles of contexts as a meaning representation (see \S\ref{subseq_intuitions_and_theory}, \S\ref{app:derivation}).


% The applicability of \method relies on contexts containing expressive information about the input to inform output $s$. 
To motivate how this method functions, consider the paraphrasing example from Figure~\ref{fig_1} with input $s_{input}:$ \textit{How are circulatory system tissues formed?} Generated contexts reflect different aspects of $s_{input}$: $c_1$ situates $s_{input}$ as a question (\textit{This is a medical question...}), while $c_2$ and $c_3$ explore central concepts  (\textit{as with all tissue...}; \textit{about the circulatory system}). Even though each context could follow many sentences, together they form a fingerprint for $s_{input}$. A sentence that could be followed by all of $c_1,c_2,c_3$ will likely be a question ($c_1$) about tissue formation ($c_2$) and the circulatory system ($c_3$), and generally occupy the same semantic neighborhood as $s_{input}$: e.g. \textit{How do circulatory systems form?}

%\peter{Then, last section connecting to infilling and other possible applications. I'm picturing this beginning something like "in paraphrasing, we are replacing all of $s_{input}$ with something that might appear in the same contexts. This is not necessary however, we might replace only part of a sentence (e.g. in context paraphrasing) or even insert text in a gap (text infilling) simply by holding part of $s_{input}$ static when we generate". Not sure if this is the best tactic though, I'm open to anything. }

In the case of paraphrasing, our task is to replace all of $s_{input}$ with something that might appear in the same contexts. Other tasks, however, might require us to replace only part of a sentence (e.g. in-context paraphrasing) or even insert text at a given position (e.g. infilling). \method makes this easy: simply hold part of $s_{input}$ static when we generate from RD.

% In the case of paraphrasing, we would like to replace the entire input. Thus, we simply sample from \rlRD (or the symmetric version, \lrRD from \S\ref{app:lr}), choosing the best output with bidirectional scoring (\S\ref{subsec:app_paraphrase}). 
% In $\alpha$NLG the input is sentences $o_1,o_2$ and the task is to generate a third sentence that \textit{bridges} the narrative gap between them. Here, the challenge for LM-decoding is making use of context from both sides ($o_1$ on the left and $o_2$ on the right). \method allows us to generate 1-sided contexts that capture information about both $o_1$ and $o_2$, then replace the 0-length gap between them by appending $o_1$ and $o_2$ to the forward and backward context ensembles, respectively (\S\ref{subsec:app_anlg}). 

\subsection{\method}
\label{subsec:reflective_decoder}

\input{figs/algorithm_simple}


% We proceed to explicitly describe the steps to generate with \method, which requires an input text $s_{input}$, as well as forward and backward language models (\lrLM and \rlLM). From \S\ref{subseq_overview}, 
% \method generates outputs that fit the same contexts as the input $s_{input}$, with the option to only overwrite a sub-span of $s_{input}$. % By first generating representative contexts, then conditioning a language model in the reverse direction under a weighted ensemble of those contexts (equation \ref{eq:RD_simple}) we define the sampling function (RD), e.g \rlRD in Algorithm~\ref{alg}.
Let's dive into the details of \method, by considering the right-hand context ensemble (\rlRD), keeping in mind that the process is repeated on the left-hand as well (\lrRD). 


First, in the \textbf{\stepone} (line 1 of Algorithm~\ref{alg}), we sample many right-hand contexts $c_i$ for $s_{input}$, using \lrLM. These will be used as a representative sample of the contexts $s_{input}$ appears in.
Second, in the \textbf{\steptwo} (lines 2 \& 3) our goal is to construct a sampling function \rlRD that will yield texts similar to $s_{input}$. We define \lrRD as:
\begin{equation}
    \text{\rlRD}(s) = \frac{ \prod_i \text{\rlLM}(s|c_i)^{w_i}}{ \prod_{j=0}^{|s|} \sum_{t \in V}  \prod_{i}  \text{\rlLM}(t|s_{j+1:|s|} + c_i)^{w_i} }
    \label{eqn:rd}
\end{equation}

\noindent
This is equivalent to equation \ref{eq:RD_simple}, but giving the exact normalization factor $Z$. 

Equation~\ref{eqn:rd} is a token-wise Product of Experts model, that captures the semantic neighborhood of $s_{input}$ via the combination of contexts $c_i$ and their weights $w_i$ (\S\ref{subseq_intuitions_and_theory}). 
We learn $w_i$ that maximize $\text{\rlRD}(s_{input})$, i.e. the probability of generating $s_{input}$. We initialize these weights (line 2),  then train them (line 3) using the Adam optimizer \citep{kingma2014adam}. We normalize weights into a proper distribution at every step (see \S\ref{app:derivation}). 

\lrRD is symmetrically learned in the reverse direction, flipping the roles of \lrLM and \rlLM and sampling left-hand context instead (see \S\ref{app:lr} for details). Finally, we generate from \rlRD (and \lrRD), sampling outputs that would appear in the same contexts as $s_{input}$. Depending on the application, we rank and select a final output in different ways, always using \lrLM and \rlLM together to capture bidirectional fit.


\input{figs/fig_examples}



\subsection{Implementation}
\label{subsec:implementation}

% Here, we cover implementation details for \S\ref{subsec:reflective_decoder}.

\paragraph{Weight Learning and Pruning} Context weights $w_i$ are learned using the Adam optimizer \citep{kingma2014adam}. In practice this takes under 100 steps (negligible time compared to LM decoding). While we sample tens of contexts (line 1 of Algorithm~\ref{alg}), many end up with negligible weight under the learned distribution (equation \ref{eqn:rd}). To efficiently sample from this function, we drop all but the top $k_c$ contexts and renormalize weights: $k_c < n_c$ contexts are used during the \steptwo.
% described in \S\ref{subsec:reflective_decoder}. 


\paragraph{Parameters} We sample $n_c$ contexts to describe the source $s_{input}$. We use nucleus sampling \citep{Holtzman2019TheCC} with parameter $p_c$, and a maximum length of $len_c$. 
% As stated in \textbf{Weight Pruning}, we drop all but the top $k_c$ contexts by weight.
Once \lrRD and \rlRD are learned, we sample $n_{s}$ generations from each, of length $len_{s}$. We again use nucleus sampling, but choose $p_{s}$ per-example to account for vastly different entropy in RD (\S\ref{app:entropy_calibtration}). Values for all hyperparameters are available in \S\ref{app:model_params}.

\paragraph{Language Models} We train large forward (\lrLM) and backward (\rlLM) language models based on GPT-2 \citep{radford2019gpt2}  using the OpenWebText training corpus \citep{Gokaslan2019OpenWeb}\footnote{https://github.com/yet-another-account/openwebtext}. Our implementation details follow those of past work retraining GPT-2 \citep{zellers2019defending}.




\subsection{Application: Paraphrasing}
\label{subsec:app_paraphrase}

%Paraphrasing is the most straightforward application for \method. \ari{The previous sentence gives you nothing.} 
To paraphrase, we begin by generating candidate outputs. Following \S\ref{subsec:reflective_decoder} the \decoder is learned in each direction (\lrRD, \rlRD) using the input sentence $s_{input}$. Then, $n_{s}$ generations are sampled from both \lrRD and \rlRD: \
$$s_1, ..., s_{n_s} \sim \text{\lrRD}, s_{n_s + 1}, ..., s_{2*n_{s} } \sim \text{\rlRD}$$
%$$\hat{s}_1, ..., \hat{s}_{n_{\hat{s}}} \sim \text{\lrRD}, \hat{s}_{n_{\hat{s}} + 1}, ..., \hat{s}_{2*n_{\hat{s}} } \sim \text{\rlRD}$$

\noindent
This gives a robust set of candidates that are compatible with the same left and right contexts as $s_{input}$. Most of these are semantically related to $s_{input}$, but must be scored and ranked in order to select true paraphrases.
% We prioritize sentences with high semantic similarity to the input. 
\method is based on a notion of similarity centered on contextual distance (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). Thus we use the sum of expectations over forward and backward context ensembles as a final scoring function, leveraging the generated contexts of \lrRD and \rlRD:
%closely related to the \method sampling function (equation \ref{eqn:rd}), which aims to give high probability to contextually similar outputs, based on contextual distance posed as cross-entropy (equation \ref{eqn:reflective_scoring} and \S\ref{subseq_intuitions_and_theory}). While the sampling function attempts to estimate this with a reverse-direction LM, for final scoring we use a more robust estimate with the original context-generating LMs:
\begin{equation}
    score(s) = \frac{1}{n_c}\sum_{c_{rh}} \text{\lrLM}(c_{rh}|s) + \frac{1}{n_c}\sum_{c_{lh}} \text{\rlLM}(c_{lh}|s)
    \label{eqn:paraphrasing_full_score}
\end{equation}
%\begin{equation}
%    score(\hat{s}) = \frac{1}{n_c}\sum_{c_{rh}} \text{\lrLM}(c_{rh}|\hat{s}) + \frac{1}{n_c}\sum_{c_{lh}} \text{\rlLM}(c_{lh}|\hat{s})
%    \label{eqn:paraphrasing_full_score}
%\end{equation}
\\
\noindent
where $c_{rh}$ are the generated contexts used in \rlRD, and $c_{lh}$ for \lrRD. This explicitly measures how well a candidate $s$ fits into the potential contexts of $s_{input}$ because it is proportional to the expectation of a given paraphrase being generated by an ensemble of those forward and backward contexts. %\peter{will expand this a little}


%\ximing{if we want to save space, can we combine equation (2) and (3)? equation (3) seems to be a pretty straightforward step}
%\noindent
%taking the highest ranked one that differs sufficiently from $s_{input}$

\subsection{Application: Abductive Reasoning}
\label{subsec:app_anlg}



Abductive natural language generation ($\alpha$NLG from \citet{Bhagavatula2019AbductiveCR}) is the task of filling in the blank between 2 observations $o1$ and $o2$, with a hypothesis $h$ that abductively explains them. The challenge for LM-decoding is making use of context from both sides ($o_1$ on the left and $o_2$ on the right). This is particularly challenging for unsupervised methods because unidirectional language models cannot naturally condition on both sides when generating $h$. 

\method simplifies this problem by generating 1-sided contexts that capture information about both $o_1$ and $o_2$, then appending $o_1$ and $o_2$ to the forward and backward context ensembles, respectively. %(\S\ref{subsec:app_anlg}). 
Concretely, we use concatenated $o_1 + o_2$ as $s_{input}$ in Algorithm~\ref{alg}, and construct sampling functions \lrRD, \rlRD informed by both observations. 
We are interested in sampling in between $o1$ and $o2$, so when sampling hypotheses $h$ from \rlRD we condition on the right-side observation $o_2$ (and vice-versa for \lrRD and $o_1$). This is equivalent to appending the given observation to sampled contexts: 
\begin{equation}
\begin{split}
    h_1, ..., h_{n_{\hat{s}}} &\sim \text{\rlRD}(h|o_2) \\ \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} &\sim \text{\lrRD}(h|o_1)
\end{split}
\end{equation}
%$$h_1, ..., h_{n_{\hat{s}}} \sim \text{\rlRD}(h|o_2) \hspace{4 pt} h_{n_{\hat{s}} + 1}, ..., h_{2*n_{\hat{s}}} \sim \text{\lrRD}(h|o_1)$$

Note that both \lrRD and \rlRD contain information about \textbf{both} $o_1$ and $o_2$, effectively turning a 2-sided contextual constraint into a 1-sided one. 

We also use a task-specific scoring function to rank sampled hypotheses. We would like a hypothesis $h$ that best explains both observations, and so use language models to measure this:
\begin{equation}
    score(h) = \text{\rlLM}(o1| h 
+ o2) + \text{\lrLM}(o2| o1 + h )
\label{eqn:anlg_score}
\end{equation}

Adding $h$ should help to ``explain'' each observation given the other, i.e. that $o2$ follows from $o1 + h$ and $o1$ from $h + o2$. To filter hypotheses that only explain one of the two observations, we remove any that make either observation less probable than the empty hypothesis, imposing:
\noindent
\begin{align*}
    \text{\rlLM}(o_1|h + o_2)>\text{\rlLM}(o_1|o_2) \\
    \text{\lrLM}(o_2|o_1 + h)>\text{\lrLM}(o_2|o_1)
\end{align*}
\subsection{Intuitions and Theory}
\label{subseq_intuitions_and_theory}
Here, we discuss the theoretical intuition for \method, as a way to sample generations that share contextual ``fit'' with a source text, deriving the sampling function of equation \ref{eqn:rd}. We start by considering how to compare a generation $s$ with an input $s_{input}$. %We focus on unsupervised paraphrasing, \peter{Should qualify this a bit more "explain in terms of", not just generally "focus on"} which requires a notion of similarity to judge whether generation $\hat{s}$ is a paraphrase of source $s_{input}$. 

For the task of paraphrasing, we follow a distributional intuition \citep{firth1957synopsis}, that textual meaning can be understood by the contexts in which text appears. Many distributional approaches learn contentful neural representations by predicting context given input text \citep{word2vec,kiros2015skip}, then compare these representations to establish semantic similarity. We can, instead, compare contexts directly—judging the difference in meaning between texts $s_{input}$ and $s$ by their divergence:
\begin{equation}
    D_{KL}(\text{\lrLM}(c|s_{input}), \text{\lrLM}(c|\hat{s}))
    \label{eqn:context_divergence}
\end{equation}
We use \lrLM to interchangeably denote the theoretical left-to-right distribution of text, and the LM estimating it. Thus, $\text{\lrLM}(c|s)$ is the distribution over right contexts $c$ given sentence s, and equation \ref{eqn:context_divergence} can be understood as the ``information difference'' we expect $s$ to have from $s_{input}$. Note, we could similarly use left-hand context and \rlLM. 

Measuring $D_{KL}$ exactly is infeasible, but for generation we are mainly interested in ranking by this score (e.g. picking the best paraphrase $s$). Thus, as in language model training—we use a finite sample estimate of cross-entropy as an effective proxy for $D_{KL}$:
\begin{equation}
\begin{split}
 \hat{H}(\text{\lrLM}(c|s_{input}), & \text{\lrLM}(c|s)) = \\ &\frac{1}{N}\sum_{c_i \sim \text{\lrLM}(c|s_{input})} -\text{log}\text{\lrLM}(c_i|s) 
 \end{split}
 \label{eqn:reflective_scoring}
 \end{equation}
Where $c_i \sim \text{\lrLM}(c|s_{input})$ indicates contexts for $s_{input}$ generated by the LM.
%This allows us to leverage high-quality generations of our pretrained LMs. 
Intuitively, we want to minimize this score when generating $s$: optimal $s$ has a similar meaning to $s_{input}$ and so fills approximately the same contextual hole as, minimizing the value of this ``contextual distance''. We explicitly test this notion for semantic equivalence in \S\ref{subsec_wmt18}.

In this form, $\hat{H}$ requires a fully generated $s$ to compare to $s_{input}$, but we are trying to \textbf{generate} $s$ for which the divergence from $s_{input}$ is low. We flip the role of ``text'' and ``context'' to define a function from which we can sample $s$: 
\begin{equation}
    \begin{split}
    &\text{\rlRD}(s_j|, s_{j+1:n}) = \frac{ \prod_i  \text{\rlLM}(s_j|s_{j+1:n} + c_i)^{w_i}}{ \sum_{t \in V}  \prod_i  \text{\rlLM}(t|s_{j+1:n} + c_i)^{w_i} }
    \end{split}
    \label{eqn:rd_theory}
\end{equation}
%\ximing{can we replace $t \in V$ with maybe $v \in V$ in equation (7) and (1)? $t$ denote timestep in many cases, we probably want to avoid it\\}
(equivalent to equation \ref{eqn:rd}, derived in \S\ref{app:derivation}) $s_j$ is the $j^{th}$ token in $s$ (sampled right-to-left from n to 0), and $V$ is the vocabulary. Weights $w_i$ are learned
%, aligning probability with contextual similarity to $s_{input}$ 
by maximizing the probability of $s_{input}$. 

Equation~\ref{eqn:rd_theory}, estimates the probability of \textit{predicting} $s_{input}$ and $s$ from a finite set of contexts $c_i$ generated from $s_{input}$. This approximately minimizes~\ref{eqn:context_divergence} because, due to the sparsity of linguistic sequences, being generated by the same weighted ensemble of contexts strongly correlates with generating the same contexts in the same proportions, i.e. low divergence.
% Thus, we induce a sequential, token-wise probability distribution that approximately minimizes . 
We can sample $s$ with low contextual distance from $s_{input}$ using \rlRD. Further, we can use left context to construct \lrRD by simply reversing the directions of the LMs used.


%\ari{We need to add more description of why the approximations (nucleus sampling forward, weight pruning backward) make sense.}

==> sections/backups/results_0.tex <==
\section{Results and Analysis}
\label{sec_results}
\label{subsec_discussion}
%\input{figs/quora_automatic_results}


%\input{figs/quora_human_eval}

\input{figs/twitter_results_small}

\paragraph{Paraphrasing} 
First, the Quora dataset: On automatic metrics from past works (BLEU, METEOR, \TERP) our lowest-$Novelty$ model setting ($\text{RD}_{Top}$) achieves the highest unsupervised scores, and highest overall on BLEU. Other high scoring rows (Source, PG-IL) are similarly low-$Novelty$. The SARI metric explicitly balances $Novelty$ with similarity to reference. On SARI we see such low-$Novelty$ models perform worse. The best overall model on SARI is our medium-$Novelty$ setting ($\text{RD}_{30}$) which outperforms MT and supervised models. 
% Our highest Novelty method ($\text{RD}_{45}$) gets within 1.5 points of this.

Our human evaluation measures what fraction of outputs are found to be fluent, consistent, and novel. As with SARI, both our mid and high-$Novelty$ models perform quite well, again with the medium-$Novelty$ setting outperforming all baselines. As further validation for SARI as a proxy for human, they share the same top-5 models. 

Results on the Twitter URL corpus largely support those on Quora. \method achieves the best unsupervised scores on novelty-aware metrics (Table~\ref{tab:twitter_results_small}), with the best overall SARI, even outperforming reference on the human metric, although MT achieves the highest overall.

In sum, \method is able to compete on previously used quality metrics favoring low-$Novelty$, but can produce more varied outputs preferred by humans. $\text{RD}_{45}$ is among the best models by SARI and Human on Quora despite exceeding the novelty of even the reference.


\paragraph{$\alpha$NLG}
Results on $\alpha$NLG (Table~\ref{tab:anlg})
present a strong case that \method{} can effectively use bidirectional context. Strong hypotheses use information from both initial the observation $o_1$ and the future observation $o_2$. Humans ranked the ability of \method{} to capture this 42.4, about 17 points above the next-best unsupervised baseline and only 15 points below the best supervised method tested. We see similar results for overall evaluation. 
A likely factor in this is the (comparatively) high degree of coherence between $h$ and $o_2$ by \method. Where other methods seem to pay more attention to observation $o_1$ (the $o_2$ column generally has much lower values), \method has comparably high coherence with left-hand ($o_1$) and right-hand ($o_2$) contexts.
%This is likely because \method excels at agreeing with the second (future) observation, $o2$, compared to recent unsupervised methods.

We also include example generations in Figure~\ref{fig_examples} to demonstrate the ability of \method to combine $o_1$ and $o_2$. For example, $h=$ \textit{He put her on the swing, and while she was on the swing, she fell off and was lying on the ground.} incorporates information from both observations. Specifically, it takes into account the swing that Ray is building for his daughter which is only mentioned in $o_1$, and hypothesizes about a potential injury due to Ray checking on his daughter in $o_2$. See appendix for more generations.

Overall, the strong performance of \method on $\alpha$NLG shows that unsupervised generation with context ensemble applies to infilling in addition to paraphrasing.
% Indeed, all we needed to apply \method was a source text whose content the generation should adhere to ($o_1$ and $o_2$ in this case), and two unidirectional LMs. 
%\ari{shorten the end of this, and save the main explanation for earlier since space is so tight}

\section{Discussion}

A major factor when considering \method is ease-of-use: armed with our pretrained language models, practitioners can immediately begin generating. The models and underlying principles apply broadly across domains making exploration and adaptation simple, no finetuning required. While multiple rounds of generation mean \method{} may run slower than other methods at inference time\footnote{Depending on parameters we found most baselines took multiple seconds per example vs. 10s of seconds for \method on a multi-gpu machine.}, it avoids training, produces high quality generations and works across domains. There are clearly settings that favor supervised learning (narrow, known domain with abundant training data), but \method is a good option to begin generating and exploring immediately. 
%Unlike other completely off-the-shelf LM solutions (e.g. few-shot GPT-3) \method can run on local GPU machines.

The algorithm and principles of \method extend beyond our experiments here, however. A simple example is in-context paraphrasing--i.e. writing a paraphrase that fits in the context that the original sentence appears in. Most existing paraphrasing methods would require significant changes to consider context as a constraint, but we can simply incorporate true context in generated contexts for \method. 
%without changing the algorithm, \method can consider both semantic similarity and contextual fit simultaneously. 
Indeed, the underlying principle of \method--that pretrained LMs naturally measure the highly semantic notion of contextual fit--is robust and natural, which is why it can be so easily extended. It can also be useful for applications beyond this generation paradigm. 
For instance, we can similarly improve the robustness of machine translation, by generating contexts for the source sentence, translating these contexts, and constraining the translation to fit the same contexts as the source. Following this line of using generated contexts to judge generations, the contextual scoring function underpinning \method{} could easily be adapted as a robust metric, with the added benefit of being differentiable. Broadly, \peter{something to try to get future work to use this paradigm}

Finally, a paragraph about non-generative, different model (``you could also use GPT-3 to score!'')

==> sections/backups/results_1.tex <==
\section{Results and Analysis}
\label{sec_results}
\label{subsec_discussion}
%\input{figs/quora_automatic_results}


%\input{figs/quora_human_eval}

\input{figs/twitter_results_small}

\paragraph{Paraphrasing} 
First, the Quora dataset: On automatic metrics from past works (BLEU, METEOR, \TERP) our lowest-$Novelty$ model setting ($\text{RD}_{Top}$) achieves the highest unsupervised scores, and highest overall on BLEU. Other high scoring rows (Source, PG-IL) are similarly low-$Novelty$. The SARI metric explicitly balances $Novelty$ with similarity to reference. On SARI we see such low-$Novelty$ models perform worse. The best overall model on SARI is our medium-$Novelty$ setting ($\text{RD}_{30}$) which outperforms MT and supervised models. 
% Our highest Novelty method ($\text{RD}_{45}$) gets within 1.5 points of this.

Our human evaluation measures what fraction of outputs are found to be fluent, consistent, and novel. As with SARI, both our mid and high-$Novelty$ models perform quite well, again with the medium-$Novelty$ setting outperforming all baselines. As further validation for SARI as a proxy for human, they share the same top-5 models. 

Results on the Twitter URL corpus largely support those on Quora. \method achieves the best unsupervised scores on novelty-aware metrics (Table~\ref{tab:twitter_results_small}), with the best overall SARI, even outperforming reference on the human metric, although MT achieves the highest overall.

In sum, \method is able to compete on previously used quality metrics favoring low-$Novelty$, but can produce more varied outputs preferred by humans. $\text{RD}_{45}$ is among the best models by SARI and Human on Quora despite exceeding the novelty of even the reference.


\paragraph{$\alpha$NLG}
Results on $\alpha$NLG (Table~\ref{tab:anlg})
present a strong case that \method{} can effectively use bidirectional context. Strong hypotheses use information from both initial the observation $o_1$ and the future observation $o_2$. Humans ranked the ability of \method{} to capture this 42.4, about 17 points above the next-best unsupervised baseline and only 15 points below the best supervised method tested. We see similar results for overall evaluation. 
A likely factor in this is the (comparatively) high degree of coherence between $h$ and $o_2$ by \method. Where other methods seem to pay more attention to observation $o_1$ (the $o_2$ column generally has much lower values), \method has comparably high coherence with left-hand ($o_1$) and right-hand ($o_2$) contexts.
%This is likely because \method excels at agreeing with the second (future) observation, $o2$, compared to recent unsupervised methods.

We also include example generations in Figure~\ref{fig_examples} to demonstrate the ability of \method to combine $o_1$ and $o_2$. For example, $h=$ \textit{He put her on the swing, and while she was on the swing, she fell off and was lying on the ground.} incorporates information from both observations. Specifically, it takes into account the swing that Ray is building for his daughter which is only mentioned in $o_1$, and hypothesizes about a potential injury due to Ray checking on his daughter in $o_2$. See appendix for more generations.

Overall, the strong performance of \method on $\alpha$NLG shows that unsupervised generation with context ensemble applies to infilling in addition to paraphrasing.
% Indeed, all we needed to apply \method was a source text whose content the generation should adhere to ($o_1$ and $o_2$ in this case), and two unidirectional LMs. 
%\ari{shorten the end of this, and save the main explanation for earlier since space is so tight}

\section{Discussion}

\paragraph{\method{} as Adaptive Prompting}
\citet{radford2019gpt2} and \citet{Brown2020LanguageMA} have popularized ``prompting'', i.e., writing a prefix to implicitly or explicitly describe a task for a generative model. This has raised interest in automatically generating such prompts \cite{shin-etal-2020-autoprompt, reynolds2021prompt} as well as going past explicit strings as prototypes \cite{Li2021PrefixTuningOC, hambardzumyan2021warp, lester2021power, qin2021learning}. In contrast, \method{} creates an ensemble of explicit prompts on both sides of an input, as a meaning representation of the span to be generated (or rewritten, in the case of paraphrasing). This can be viewed as adaptively prompting the left and right language models, to capture the desiderata for the generation, which our results show effectively capture bidirectional context.


\paragraph{Out-of-the-Box Application}
A major advantage to \method is ease-of-use: armed with our pretrained language models, practitioners can immediately begin generating. The models and principles underlying the method apply broadly across domains, making exploration and adaptation simple, no finetuning required. While multiple rounds of generation mean \method{} may run slower than other methods at inference time\footnote{Depending on parameters we found most baselines took multiple seconds per example vs. 10s of seconds for \method on a multi-gpu machine.} it avoids training, produces high quality generations and works across domains. There are clearly settings that favor supervised learning (narrow, known domain with abundant training data), but \method is a good option to begin generating and exploring immediately. 

\paragraph{Future Applications}
%Unlike other completely off-the-shelf LM solutions (e.g. few-shot GPT-3) \method can run on local GPU machines.

The algorithm and principles of \method extend beyond our experiments here, however. A simple example is in-context paraphrasing--i.e. writing a paraphrase that fits in the context that the original sentence appears in. Most existing paraphrasing methods would require significant changes to consider context as a constraint, but we can simply incorporate true and generated contexts for \method. 
%without changing the algorithm, \method can consider both semantic similarity and contextual fit simultaneously. 
Indeed, the underlying principle of--that pretrained LMs naturally measure the highly semantic notion of contextual fit--is robust, which is why it can be so easily extended. It can be useful for applications beyond this generation paradigm. 
For instance, we can similarly improve the robustness of machine translation, by generating contexts for the source sentence, translating these contexts, and constraining the translation to fit the same contexts as the source. This principle is not tied to generation or the models used here, however; a strong semantic similarity score could be attained by measuring the contextual fit function (Equation~\ref{eqn:reflective_scoring}) with a very large pretrained language model like GPT-3. There are countless applications in any domain where semantic notions are needed and language models are available. 

\paragraph{Span Representations with Unidirectional LMs}
To get the representation of a span, most NLP researchers and practitioners use a Masked LM (MLM), which is trained to predict masked-out tokens and thus uses bidirectional context. However, Unidirectional LMs implicitly contain an MLM distribution. For instance, given a prefix $p$ and a suffix $s$ we could get predictions for the ``masked'' token $m$ in between them using $p(m=t|p,s) = \frac{P(s|p,t)}{\sum_{v\in V}P(s|p,v)}$ where $V$ is the vocabulary. This is a token-level application of the fact that Unidirectional LMs implicitly capture a density function across all strings, and thus contain information about how likely any span is in any context, even a bidirectional context.

\method{} takes advantage of this implicit span representation to get explicit representations by generating and re-weighting an ensemble of contexts. For paraphrasing (\S\ref{subsec:app_paraphrase}) we get the representation of an observed span, while for $\alpha$NLG (\S\ref{subsec:app_anlg}) we use \method{} to get a representation for an unobserved span. The fact that Unidirectional LMs are actually just left-to-right factored density functions gives us enormous flexibility, and one that is only beginning to be untapped since most tasks only require a left-to-right generation or a decision for a single token or sentence.

==> sections/backups/results_2.tex <==
\section{Results and Analysis}
\label{sec_results}
\label{subsec_discussion}
%\input{figs/quora_automatic_results}


%\input{figs/quora_human_eval}

\input{figs/twitter_results_small}

\paragraph{Paraphrasing} 
First, the Quora dataset: On automatic metrics from past works (BLEU, METEOR, \TERP) our lowest-$Novelty$ model setting ($\text{RD}_{Top}$) achieves the highest unsupervised scores, and highest overall on BLEU. Other high scoring rows (Source, PG-IL) are similarly low-$Novelty$. The SARI metric explicitly balances $Novelty$ with similarity to reference. On SARI we see such low-$Novelty$ models perform worse. The best overall model on SARI is our medium-$Novelty$ setting ($\text{RD}_{30}$) which outperforms MT and supervised models. 
% Our highest Novelty method ($\text{RD}_{45}$) gets within 1.5 points of this.

Our human evaluation measures what fraction of outputs are found to be fluent, consistent, and novel. As with SARI, both our mid and high-$Novelty$ models perform quite well, again with the medium-$Novelty$ setting outperforming all baselines. As further validation for SARI as a proxy for human, they share the same top-5 models. 

Results on the Twitter URL corpus largely support those on Quora. \method achieves the best unsupervised scores on novelty-aware metrics (Table~\ref{tab:twitter_results_small}), with the best overall SARI, even outperforming reference on the human metric, although MT achieves the highest overall.

In sum, \method is able to compete on previously used quality metrics favoring low-$Novelty$, but can produce more varied outputs preferred by humans. $\text{RD}_{45}$ is among the best models by SARI and Human on Quora despite exceeding the novelty of even the reference.


\paragraph{$\alpha$NLG}
Results on $\alpha$NLG (Table~\ref{tab:anlg})
present a strong case that \method{} can effectively use bidirectional context. Strong hypotheses use information from both initial the observation $o_1$ and the future observation $o_2$. Humans ranked the ability of \method{} to capture this 42.4, about 17 points above the next-best unsupervised baseline and only 15 points below the best supervised method tested. We see similar results for overall evaluation. 
A likely factor in this is the (comparatively) high degree of coherence between $h$ and $o_2$ by \method. Where other methods seem to pay more attention to observation $o_1$ (the $o_2$ column generally has much lower values), \method has comparably high coherence with left-hand ($o_1$) and right-hand ($o_2$) contexts.
%This is likely because \method excels at agreeing with the second (future) observation, $o2$, compared to recent unsupervised methods.

We also include example generations in Figure~\ref{fig_examples} to demonstrate the ability of \method to combine $o_1$ and $o_2$. For example, $h=$ \textit{He put her on the swing, and while she was on the swing, she fell off and was lying on the ground.} incorporates information from both observations. Specifically, it takes into account the swing that Ray is building for his daughter which is only mentioned in $o_1$, and hypothesizes about a potential injury due to Ray checking on his daughter in $o_2$. See appendix for more generations.

Overall, the strong performance of \method on $\alpha$NLG shows that unsupervised generation with context ensemble applies to infilling in addition to paraphrasing.
% Indeed, all we needed to apply \method was a source text whose content the generation should adhere to ($o_1$ and $o_2$ in this case), and two unidirectional LMs. 
%\ari{shorten the end of this, and save the main explanation for earlier since space is so tight}

\section{Discussion}

\paragraph{\method{} as Adaptive Prompting}
\citet{radford2019gpt2} and \citet{Brown2020LanguageMA} have popularized ``prompting'', i.e., writing a prefix to implicitly or explicitly describe a task for a generative model. This has raised interest in automatically generating such prompts \cite{shin-etal-2020-autoprompt, reynolds2021prompt} as well as going past explicit strings as prototypes \cite{Li2021PrefixTuningOC, hambardzumyan2021warp, lester2021power, qin2021learning}. In contrast, \method{} creates an ensemble of explicit prompts on both sides of an input, as a meaning representation of the span to be generated (or rewritten, in the case of paraphrasing). This can be viewed as adaptively prompting the left and right language models, to capture the desiderata for the generation, which our results show effectively capture bidirectional context.


\paragraph{Out-of-the-Box Application}
A major advantage to \method is ease-of-use: armed with our pretrained language models, practitioners can immediately begin generating. The models and principles underlying the method apply broadly across domains, making exploration and adaptation simple, no finetuning required. While multiple rounds of generation mean \method{} may run slower than other methods at inference time\footnote{Depending on parameters we found most baselines took multiple seconds per example vs. 10s of seconds for \method on a multi-gpu machine.} it avoids training, produces high quality generations and works across domains. There are clearly settings that favor supervised learning (narrow, known domain with abundant training data), but \method is a good option to begin generating and exploring immediately. 

\paragraph{Future Applications}
%Unlike other completely off-the-shelf LM solutions (e.g. few-shot GPT-3) \method can run on local GPU machines.

The algorithm and principles of \method extend beyond our experiments here, however. A simple example is in-context paraphrasing--i.e. writing a paraphrase that fits in the context that the original sentence appears in. Most existing paraphrasing methods would require significant changes to consider context as a constraint, but we can simply incorporate true and generated contexts for \method. 
%without changing the algorithm, \method can consider both semantic similarity and contextual fit simultaneously. 
Indeed, the underlying principle of--that pretrained LMs naturally measure the highly semantic notion of contextual fit--is robust, which is why it can be so easily extended. It can be useful for applications beyond this generation paradigm. 
For instance, we can similarly improve the robustness of machine translation, by generating contexts for the source sentence, translating these contexts, and constraining the translation to fit the same contexts as the source. This principle is not tied to generation or the models used here, however; a strong semantic similarity score could be attained by measuring the contextual fit function (Equation~\ref{eqn:reflective_scoring}) with a very large pretrained language model like GPT-3. There are countless applications in any domain where semantic notions are needed and language models are available. 

\paragraph{Span Representations with Unidirectional LMs}
To get the representation of a span, most NLP researchers and practitioners use a Masked LM (MLM), which is trained to predict masked-out tokens and thus uses bidirectional context. However, Unidirectional LMs implicitly contain an MLM distribution. For instance, given a prefix $p$ and a suffix $s$ we could get predictions for the ``masked'' token $m$ in between them using $p(m=t|p,s) = \frac{P(s|p,t)}{\sum_{v\in V}P(s|p,v)}$ where $V$ is the vocabulary. This is a token-level application of the fact that Unidirectional LMs implicitly capture a density function across all strings, and thus contain information about how likely any span is in any context, even a bidirectional context.

\method{} takes advantage of this implicit span representation to get explicit representations by generating and re-weighting an ensemble of contexts. For paraphrasing (\S\ref{subsec:app_paraphrase}) we get the representation of an observed span, while for $\alpha$NLG (\S\ref{subsec:app_anlg}) we use \method{} to get a representation for an unobserved span. The fact that Unidirectional LMs are actually just left-to-right factored density functions gives us enormous flexibility, and one that is only beginning to be untapped since most tasks only require a left-to-right generation or a decision for a single token or sentence.
